QUAR-VLA: Vision-Language-Action Model for Quadruped Robots

The important manifestation of robot intelligence is the ability to naturally interact and autonomously make decisions. Traditional approaches to robot control often compartmentalize perception, planning, and decision-making, simplifying system design but limiting the synergy between different information streams. This compartmentalization poses challenges in achieving seamless autonomous reasoning, decision-making, and action execution. To address these limitations, a novel paradigm, named Vision-Language-Action tasks for QUAdruped Robots (QUAR-VLA), has been introduced in this paper. This approach tightly integrates visual information and instructions to generate executable actions, effectively merging perception, planning, and decision-making. The central idea is to elevate the overall intelligence of the robot. Within this framework, a notable challenge lies in aligning fine-grained instructions with visual perception information. This emphasizes the complexity involved in ensuring that the robot accurately interprets and acts upon detailed instructions in harmony with its visual observations. Consequently, we propose QUAdruped Robotic Transformer (QUART), a family of VLA models to integrate visual information and instructions from diverse modalities as input and generates executable actions for real-world robots and present QUAdruped Robot Dataset (QUARD), a large-scale multi-task dataset including navigation, complex terrain locomotion, and whole-body manipulation tasks for training QUART models. Our extensive evaluation (4000 evaluation trials) shows that our approach leads to performant robotic policies and enables QUART to obtain a range of emergent capabilities.

==> paper/04a_Experiments_Datasets.tex <==
\vspace{-.2em}
\label{sec:experimentsdatasetes}











==> paper/06_LimSocDis.tex <==
% \vspace{-1.5em}
\section{Limitations} \label{sec:limitations}
% 1.目前模型的推理速度太慢了，在四组机器人的控制任务中需要更高地控制频率才可以保证四足机器人控制的效果。后续，我们将对模型进行量化加速，减小模型的推理时间，从而实现更高频率的控制。
% 2.当前模型的训练数据中真实数据占比太少了。因此，我们后续会考虑提出一种自动化数据采集的方式，来提高真实环境数据的采集效率。
% 3.没有把本体数据考虑进推理过程中，不利于对于四足机器人进行更精细地控制。后续我们将进一步研究如何将四足机器人的本体数据考虑进来，提出一个更加完善的模型。
% 1. Currently, the inference speed of the model is too slow, requiring a higher control frequency in the control tasks of the four robot groups to ensure effective control of the quadruped robots. In the future, we will implement quantized acceleration on the model to reduce the inference time, thus achieving higher-frequency control.

% 2. The proportion of real data in the current model's training data is too low. Consequently, we plan to explore an automated data collection method to improve the efficiency of gathering real-world environment data.

% 3. The omission of body data in the inference process hinders precise control of the quadruped robot. In subsequent studies, we will investigate incorporating body data for a more refined control and propose a more comprehensive model.

\textbf{Inefficiency in Data Collection}: Our process of data collection has been notably inefficient, leaving room for significant expansion in both the scale and diversity of our data in the future. Moving forward, it is essential to design more automated and expedited methods for data collection. Employing strategies, including but not limited to active learning and data augmentation, will facilitate the expansion of our dataset, laying the groundwork for a more comprehensive and robust dataset.

\textbf{Persisting Sim2Real Gap Issues}: While we have achieved commendable results in simulations, a noticeable gap remains between these environments and real-world applications. Therefore, rather than relying solely on straightforward co-training, it is imperative to adopt more adaptive and generalized approaches to bridge this gap. Strategies such as data augmentation, improved modeling of physics engines, or domain randomization are critical in overcoming these discrepancies.

\textbf{Need for Improved Inference Speed}: Currently, our large models achieve an inference speed of 2Hz, which is still far from matching the performance of traditional control methods employed in robotics. In the future, we aim to explore superior model compression techniques and hardware acceleration technologies to enhance the efficiency of our models significantly. By doing so, we strive to narrow the gap and ensure our models perform more effectively in real-time applications.

\textbf{Neglect of Body Data in Inference}: The exclusion of body data from the inference process significantly compromises the precision of controlling quadruped robots. Future studies are committed to incorporating body data to achieve more refined control mechanisms. This endeavor aims to develop a more comprehensive model that integrates body dynamics, enhancing the accuracy and responsiveness of quadruped robots in diverse operational scenarios.

% Firstly, the inference speed of our proposed \textbf{QUART} is too slow, requiring a higher control frequency in the control tasks of the four robot groups to ensure effective control of the quadruped robots. In the future, we will implement quantized acceleration on the model to reduce the inference time, thus achieving higher-frequency control. Secondly, the proportion of real data in the current model's training data is too low. Next, we plan to explore an automated data collection method to improve the efficiency of gathering real-world environment data. Finally, the omission of body data in the inference process hinders precise control of the quadruped robot. In subsequent studies, we will investigate incorporating body data for a more refined control and propose a more comprehensive model.

% Firstly, the inference speed of our proposed QUART is too slow, requiring a higher control frequency in the control tasks of the four robot groups to ensure effective control of the quadruped robots. In the future, we will implement quantized acceleration on the model to reduce the inference time, thus achieving higher-frequency control. Secondly, the proportion of real data in the current model's training data is too low. Next, we plan to explore an automated data collection method to improve the efficiency of gathering real-world environment data. Finally, the omission of body data in the inference process hinders precise control of the quadruped robot. In subsequent studies, we will investigate incorporating body data for a more refined control and propose a more comprehensive model.
% \px{
% \vspace{-1em}
% \textbf{Modeling the Perception of Dynamic Environments.} One important aspect for future work is to focus on developing models that can effectively perceive and adapt to dynamic environments in real-time. This entails incorporating techniques such as object tracking and motion prediction to enhance the robot's ability to understand and respond to changes in its surroundings.
% \textbf{Automated Data Collection for Larger Datasets.} To overcome the challenge of limited training data, future work can explore automated processes for data collection. This may involve leveraging robotic systems equipped with sensors to gather data from a variety of scenarios and environments. Additionally, techniques such as active learning and data augmentation can be employed to further expand the dataset size and diversity.
% \textbf{Modeling Multimodal Relationships for Enhanced Perception.} Enhancing the model's perception capabilities can be achieved by exploring the relationships and interactions between different modalities, such as vision, language, and proprioception. Future work can focus on developing novel architectures that effectively fuse and leverage information from multiple modalities to improve the robot's perception and understanding of the environment.
% \textbf{Improving Inference Speed for Real-time Control.} To address the control frequency issue, future work should aim to optimize the inference speed of VLA models. This can involve exploring hardware acceleration techniques, such as specialized processors or parallel computing architectures, to enable faster and more efficient execution of the models.
% % }

% \pagebreak

==> paper/TODO.tex <==


1. 标题是QUAR-VLA: Vision-Language-Action Model for Quadruped Robots， 感觉这里的Model不是很合适

2. Introduction的第二段提到的内容，comnimational commands; complex spatial relationships, commonsense command priors, 这些东西并没有在文章中体现
这些部分说的多一点！！！！！！！！！！！！！！
这样的话是不是对应图1部分的语言指令也要换一下

3. 任务是递进的？平行的？

TODO:

1. Introduction 部分的写作逻辑（鹏翔）

2. related work里面，参考文献的添加，robotdata的重新整理（文轩）

3. Method的overview的图（文杰）
    要体现执行频率上的问题

4. Method部分的data collection（赵晗）
   Method部分的data 展现图：七种任务+真实任务中第三视角的轨迹图（鹏翔+文杰）

5. Method部分的data analysis(柠溪)

6. Method部分的model的设计QUART-1 （鹏翔），方法论的重新排版（感觉来不及的话就不用排版了）

   Method部分的model的设计QUART-2 （鹏翔）
   强调视觉端的GAP不大（需要用一个Fuyu的VQA任务去讲），我觉得可以直接用NaVID的结论使用，不用自己去证明

7. Method部分对于感知频率和执行频率的解释，如何实现由感知到最终实行动作的

8. 实验部分baseline的挑选：VLM+ policy的范式,  RT-2(freeze) 和 RT-1(freeze)， RT-2，

8. 实验部分的表格，分为仿真中multi-task的比对（鹏翔）200
                    仿真中unseen object的结果
                    仿真中unseen verbal的结果
   
9. 实验部分的表格，分为真实中multi-task的比对（鹏翔）20
                    仿真中unseen object的结果
                    仿真中unseen verbal的结果
                    真实中unseen background的结果

10. 涌现能力：comnimational commands; complex spatial relationships, commonsense command priors（鹏翔）

11.训练范式的消融：
    scale of data

12. 可视化实验：（文杰/鹏翔/柠溪）
    双栏（仿真中第一和第三视角的结果），7个任务
    
    




==> supmat/first_section.tex <==
\vspace{-1.5cm}
\begin{center}
\begin{large}
  \textbf{Abstract}
\vspace{-.2cm}  
\end{large}
\end{center}
\vspace{-.2cm}
\small
This supplementary material provides more information and additional experiments that could not be included in the main article due to space limitations. The document is organized as:
\vspace{-.1cm}
\begin{itemize}
\item[$\bullet$] In (\textbf{Sec: 1. Details of QUART}), we show more details of the data model structure and training strategy. 
\end{itemize}
\vspace{-.4cm}

\begin{itemize}
\item[$\bullet$] In (\textbf{Sec: 3. More results}), we provide additional results of the .
\end{itemize}




%%%%%%%%%%%%%%%%%%%










==> supmat/table_s_ab1.tex <==
% 需要添加更多的指标,比如说拿出几个类别作为例子，剩下类别的结果放在补充材料上

% 60 Intra-encoder: 9
% 61 Intra-encoder: 6
% 62 Intra-encoder: 3
% 63 Intra-encoder: 15
% 64 ca_layer:2
% 65 ca_layer:3
% 66 ca_layer:4
% 67 ca_layer:6
% 68 predictor mlp:2
% 69 predictor mlp:3
% 70 predictor gcn
% 71 intra-encoder: st-transformer

\begin{table}[!ht]
\scriptsize
\renewcommand\arraystretch{1.2}% 行距
\centering
\caption{{Ablation experiments on the GCN numbers of intra-context encoder.} 
}
\vspace{-1em}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|ccccc|cccc}
\hline
 {Num of GCN} &{3}&{6} & {9} & {12} & {15}    &0.2s  & 0.4s  & 0.8s  & 1.0s   
\\ 
\hline
\cellcolor{white} &{\checkmark} &  & & &   &{16.5} &{42.1} &93.4 &113.7    
\\
\cellcolor{white}& &\checkmark  &  &&   &{16.4} &41.5 &{92.7} &{112.5}  
\\
\cellcolor{white}& &  &\checkmark  & &  &\textbf{16.3} &\textbf{40.4} &{89.2} &{109.4}  
\\
\multirow{-3}{*}{{\cellcolor{white}\textbf{Variants}}}
{\cellcolor{white}} 
& &  & & & \checkmark  &{16.2} &40.7 &89.1 &107.6 \\ 
            
\hline
{\textbf{EAI}}& &  &  & \checkmark &  & {16.7} & {40.7} & \textbf{85.8} & \textbf{104.6}  \\
\bottomrule
\end{tabular}
}
\vspace{-0.25cm}
\label{tab:s_ab_gcnnum}
\end{table}


==> supmat/table_s_ab2.tex <==
% 需要添加更多的指标,比如说拿出几个类别作为例子，剩下类别的结果放在补充材料上

% 60 Intra-encoder: 9
% 61 Intra-encoder: 6
% 62 Intra-encoder: 3
% 63 Intra-encoder: 15
% 64 ca_layer:2
% 65 ca_layer:3
% 66 ca_layer:4
% 67 ca_layer:6
% 68 predictor mlp:2
% 69 predictor mlp:3
% 70 predictor gcn
% 71 intra-encoder: st-transformer
\vspace{-.2cm}
\begin{table}[!ht]
\scriptsize
\renewcommand\arraystretch{1.2}% 行距
\centering
\caption{{Ablation experiments of cross-attention module.} 
}
\vspace{-1em}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|ccccc|cccc}
\hline
 {Num of CA} &{2}&{3} & {4} & {5} & {6}    &0.2s  & 0.4s  & 0.8s  & 1.0s   
\\ 
\hline
\cellcolor{white} &{\checkmark} &  & & &   &\textbf{16.5} &43.3 &94.6 &112.0  
\\
\cellcolor{white}& &\checkmark  &  &&  &{16.6} &42.7 &{93.4} &{112.9}  
\\
\cellcolor{white}& &  &\checkmark  & &  &{16.6} &42.2 &90.8 &109.4 
\\
\multirow{-3}{*}{{\cellcolor{white}\textbf{Variants}}}
{\cellcolor{white}} 
& &  & & & \checkmark  &{16.8} &41.3 &{89.6} &{109.1}    \\ 
            
\hline
{\textbf{EAI}}& &  &  & \checkmark &  & {16.7} & \textbf{40.7} & \textbf{85.8} & \textbf{104.6} \\
\bottomrule
\end{tabular}
}
\vspace{-0.25cm}
\label{tab:s_ab_canum}
\end{table}


==> supmat/table_s_ab3.tex <==
% 需要添加更多的指标,比如说拿出几个类别作为例子，剩下类别的结果放在补充材料上

% 60 Intra-encoder: 9
% 61 Intra-encoder: 6
% 62 Intra-encoder: 3
% 63 Intra-encoder: 15
% 64 ca_layer:2
% 65 ca_layer:3
% 66 ca_layer:4
% 67 ca_layer:6
% 68 predictor mlp:2
% 69 predictor mlp:3
% 70 predictor gcn
% 71 intra-encoder: st-transformer
\vspace{-.2cm}
\begin{table}[!ht]
\scriptsize
\renewcommand\arraystretch{1.2}% 行距
\centering
\caption{{Ablation experiments of predictor.} 
}
% \vspace{-1em}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|cccc|cccc}
\hline
 {} &{1-MLP} &{2-MLPs}&{3-MLPs} & {GCN}   &0.2s  & 0.4s  & 0.8s  & 1.0s 
\\ 
\hline
\cellcolor{white} & & {\checkmark} & &   &{17.0} &{40.9} &86.5 &107.6 
\\
\cellcolor{white}& &  & {\checkmark} &   &{17.8} &\textbf{40.3} &{86.3} &{107.0}  
\\
\multirow{-3}{*}{{\cellcolor{white}\textbf{Variants}}}
\cellcolor{white}& &  &  &{\checkmark}   &\textbf{16.6} &41.9 &{92.6} &{114.4} 
\\

           
\hline
{\textbf{EAI}}&\checkmark &   &  &  & {16.7} & {40.7} & \textbf{85.8} & \textbf{104.6}  \\
\bottomrule
\end{tabular}
}
% \vspace{-0.1cm}
\label{tab:s_ab_pred}
\end{table}


==> supmat/table_s_ab4.tex <==
% 需要添加更多的指标,比如说拿出几个类别作为例子，剩下类别的结果放在补充材料上

% 60 Intra-encoder: 9
% 61 Intra-encoder: 6
% 62 Intra-encoder: 3
% 63 Intra-encoder: 15
% 64 ca_layer:2
% 65 ca_layer:3
% 66 ca_layer:4
% 67 ca_layer:6
% 68 predictor mlp:2
% 69 predictor mlp:3
% 70 predictor gcn
% 71 intra-encoder: st-transformer

\vspace{-.2cm}
\begin{table}[!ht]
\scriptsize
\renewcommand\arraystretch{1.2}% 行距
\centering
\caption{{Ablation experiments of intra-context encoder types.} 
}
\vspace{-1em}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|cc|cccc}
\hline
 {Type of Intra-encoder} &{GCN}&{ST-Transformer}    &0.2s  & 0.4s  & 0.8s  & 1.0s   
\\ 
\hline
\multirow{-1}{*}{{\cellcolor{white}\textbf{Variants}}}
\cellcolor{white} & & {\checkmark}   &{17.4} &{43.7} &90.4 &109.8 
\\
            
\hline
{\textbf{EAI}} & \checkmark &  & \textbf{16.7} & \textbf{40.7} & \textbf{85.8} & \textbf{104.6} \\
\bottomrule
\end{tabular}
}
\vspace{-0.25cm}
\label{tab:s_ab_intra}
\end{table}


==> supmat/table_s_ab_g.tex <==

\begin{table}[htb]
\vspace{-.em}
\caption{{Generalization experiment on AMASS.} }
\label{tab:r_amass}
\vspace{-.8em}
\renewcommand\arraystretch{1.2}% 行距
\footnotesize
\centering
\setlength{\tabcolsep}{3mm}{
\begin{tabular}{cc|cccc}
% \multicolumn{2}{c|}{} &\multicolumn{4}{c}{whole-body} \\
\hline
\multicolumn{2}{c|}{Time (sec)}     & 0.2 & 0.4  & 0.8  & 1.0\\  
\hline
 & {LTD (U)}	
&21.5  &55.8  &86.1 &117.5 \\
& {SPGSN (U)} 
&21.8 &55.3 &79.7  &110.8 \\

 
\hline
& {\textbf{EAI} (Ours)}
						 		
&\textbf{19.5  } &\textbf{55.0}&\textbf{76.5} &\textbf{102.6 }\\
\bottomrule
\end{tabular}
}
\vspace{-.5em}
\end{table}

==> supmat/table_s_arch.tex <==
\begin{table*}[t]
\scriptsize
\renewcommand\arraystretch{1.2}% 行距
\centering
\caption{Details of Architecture. }
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{@{}cccc@{}}
\toprule
layer name       & input size                              & hyperparameters                                                                                                                                                                                                                                              & output size     \\ \midrule
DCT              & (75/45/45)×T                            &                                                                                                                                                                                                                                                              & (75/45/45)×$H_c$ \\\midrule
Replicate        & (75/45/45)×$H_c$                         &                                                                                                                                                                                                                                                              & (75/48/48)×$H_c$ \\\midrule
GCN\_1           & (75/48/48)×$H_c$                         & \begin{tabular}[c]{@{}c@{}}Graph 75×75/48×48/48×48, H;\\ BN,Tanh,Dropout\end{tabular}                                                                                                                                                                     & (75/48/48)×H    \\\midrule
12 GCN\_Blocks   & (75/48/48)×H                            & \begin{tabular}[c]{@{}c@{}}Graph 75×75/48×48/48×48, H;\\ BN, Tanh, Dropout;\\ Graph 75×75/48×48/48×48, H;\\ BN, Tanh, Dropout;\\ ...(×12)\\ Graph 75×75/48×48/48×48, H;\\ BN, Tanh, Dropout;\\ Graph 75×75/48×48/48×48, H;\\ BN, Tanh, Dropout;\end{tabular} & (75/48/48)×H    \\\midrule
DN\_ml           & 75×H; 48×H                              &                                                                                                                                                                                                                                                              & 75×H; 48×H      \\\midrule
DN\_mr           & 75×H; 48×H                              &                                                                                                                                                                                                                                                              & 75×H; 48×H      \\\midrule
DN\_rl           & 48×H; 48×H                              &                                                                                                                                                                                                                                                              & 48×H; 48×H      \\\midrule
5 SI\_Blocks\_ml & 75×H; 48×H                              & \begin{tabular}[c]{@{}c@{}}Attention, Add\&LN;\\ Linear(H×4H), ReLU, Dropout, Linear(4H×H), Dropout\\ …(×5)\\ Attention, Add\&LN;\\ Linear(4H×H), ReLU, Dropout, Linear(4H×H)\end{tabular}                                                                & 75×H            \\\midrule
5 SI\_Blocks\_mr & 75×H; 48×H                              & \begin{tabular}[c]{@{}c@{}}Attention, Add\&LN;\\ Linear(H×4H), ReLU, Dropout, Linear(4H×H) , Dropout\\ …(×5)\\ Attention, Add\&LN;\\ Linear(4H×H), ReLU, Dropout, Linear(4H×H)\end{tabular}                                                                & 75×H            \\\midrule
5 SI\_Blocks\_lm & 48×H;75×H                               & \begin{tabular}[c]{@{}c@{}}Attention, Add\&LN;\\ Linear(H×4H), ReLU, Dropout, Linear(4H×H) , Dropout\\ …(×5)\\ Attention, Add\&LN;\\ Linear(4H×H), ReLU, Dropout, Linear(4H×H)\end{tabular}                                                                & 48×H            \\\midrule
5 SI\_Blocks\_lr & 48×H; 48×H                              & \begin{tabular}[c]{@{}c@{}}Attention, Add\&LN;\\ Linear(H×4H), ReLU, Dropout, Linear(4H×H) , Dropout\\ …(×5)\\ Attention, Add\&LN;\\ Linear(4H×H), ReLU, Dropout, Linear(4H×H)\end{tabular}                                                                & 48×H            \\\midrule
5 SI\_Blocks\_rm & 48×H;75×H                               & \begin{tabular}[c]{@{}c@{}}Attention, Add\&LN;\\ Linear(H×4H), ReLU, Dropout, Linear(4H×H) , Dropout\\ …(×5)\\ Attention, Add\&LN;\\ Linear(4H×H), ReLU, Dropout, Linear(4H×H)\end{tabular}                                                                & 48×H            \\\midrule
5 SI\_Blocks\_rl & 48×H; 48×H                              & \begin{tabular}[c]{@{}c@{}}Attention, Add\&LN;\\ Linear(H×4H), ReLU, Dropout, Linear(4H×H) , Dropout\\ …(×5)\\ Attention, Add\&LN;\\ Linear(4H×H), ReLU, Dropout, Linear(4H×H)\end{tabular}                                                                & 48×H            \\\midrule
Concat           & (75/48/48)×H;(75/48/48)×H;(75/48/48)×H; &                                                                                                                                                                                                                                                              & (75/48/48)×3H   \\\midrule
PI\_Block\_rm    & 75×3H;48×3H                             & Linear(H×H×1), Weighted Sum                                                                                                                                                                                                                                  & 75×3H;45×3H     \\\midrule
PI\_Block\_lm    & 75×3H;48×3H                             & Linear(H×H×1), Weighted Sum                                                                                                                                                                                                                                  & 75×3H;45×3H     \\ \midrule
MLP              & (75/45/45)×3H                           & Linear(3H×$H_c$)                                                                                                                                                                                                                                              & (75/45/45)×$H_c$ \\\midrule
IDCT             & (75/45/45)×$H_c$                         &                                                                                                                                                                                                                                                              & (75/45/45)×$\Delta T$\\ \bottomrule  
\end{tabular}
}
\label{Table:arch}
\end{table*}

==> supmat/table_s_lefthand.tex <==
% SPGSN (AW)的结果和Wholebody的结果都需要更新，正在跑

% 30 没有A（w/o MMD loss; w/o DN）
% 31 # 没有A（w MMD loss; w/o DN）
% 32 没有A（w/0 MMD loss; w DN）
% 33  没有I（w/0 Phy; w/0 S）
% 34  没有I（w/0 Phy; w S）
% 35  没有I（w Phy; w/o S）

% 30 没有A,没有I（w/o MMD loss; w/o DN）
% 
%  \textbf{(3)} As to the key components of our method, we can observe that XCI is the most important design. With the help of XCA, the extracted interaction information is more expressive and lead to more high-fidelity prediction.

\begin{table}[t]
% \vspace{-1.5em}
\caption{{Average results of left hand with finer intervals.} }
\label{tab:s_lh}
\vspace{-.7em}
\renewcommand\arraystretch{1.3}% 行距
\scriptsize
\centering
%cell大小
% \setlength{\aboverulesep}{1.85mm}
% \setlength{\belowrulesep}{-0.05mm}
\setlength{\tabcolsep}{0.7mm}{
\begin{tabular}{cc|cccccccccc}
\hline
 \multicolumn{2}{c|}{} &\multicolumn{10}{c}{Left Hand}\\
% \hline
\multicolumn{2}{c|}{Time (sec)}     & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8  & 0.9 & 1.0        \\
\hline
& LTD (D)~\cite{mao2019learning}

&7.4 &19.7 &37.0 &57.0 &78.0 &99.5 &121.4 &143.2 &163.1 &181.5

\\
% & DMGNN (D)~\cite{li2020dynamic}  
% & &24.8 & &62.0 &  & & &153.2 & &190.1
% % &23.0  &55.7  &107.7  &131.4
% \\
% &{PGBIG (D)~\cite{ma2022progressively}} 

% & &22.8 & &61.5 &  & & &149.9 & &186.7
% \\
% 右手的结果需要更新
\multirow{-4}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{}}}
& {SPGSN (D)~\cite{li2022skeleton}}

&10.1 &25.3 &42.9 &61.1 &78.1  &94.5 &111.9 &129.8 &147.3 &164.2


\\

\hline
\hline
% RH 结果有点问题，需要重新训练
{\cellcolor{white}} & {\cellcolor{white}LTD (U)~\cite{mao2019learning}}

&8.0 &19.9 &34.7 &50.5&66.5 &83.8 &103.0 &123.4&143.6 &162.5\\

% & DMGNN (D)~\cite{li2020dynamic}  

% & &22.4 & &57.3 &  & & &141.1 & &172.0
% \\
% &{PGBIG (D)~\cite{ma2022progressively}} 

% & &23.0 & &56.4 &  & & &130.4 & &165.7
% \\
{\cellcolor{white}} & {SPGSN (U)~\cite{li2022skeleton}}   

&8.6 &21.6 &38.3 &55.5 &72.9 &90.0 &108.1 &126.0 &143.0 &161.6\\

\hline
\hline

\multirow{-7}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{}}}


& {\cellcolor{white}\textbf{EAI} (Ours)}

&\textbf{6.1} &\textbf{17.7} &\textbf{33.1} &\textbf{49.2}&\textbf{64.6} &\textbf{79.4} &\textbf{94.5} &\textbf{110.1}&\textbf{124.0} &\textbf{136.4}
\\
\bottomrule

\end{tabular}
}
\vspace{-.5em}
\end{table}

==> supmat/table_s_mainbody.tex <==
% SPGSN (AW)的结果和Wholebody的结果都需要更新，正在跑

% 30 没有A（w/o MMD loss; w/o DN）
% 31 # 没有A（w MMD loss; w/o DN）
% 32 没有A（w/0 MMD loss; w DN）
% 33  没有I（w/0 Phy; w/0 S）
% 34  没有I（w/0 Phy; w S）
% 35  没有I（w Phy; w/o S）

% 30 没有A,没有I（w/o MMD loss; w/o DN）
% 
%  \textbf{(3)} As to the key components of our method, we can observe that XCI is the most important design. With the help of XCA, the extracted interaction information is more expressive and lead to more high-fidelity prediction.

\begin{table}[h]
% \vspace{-1.5em}
\caption{{Average results of major body with finer intervals.} }
\label{tab:s_mb}
\vspace{-.7em}
\renewcommand\arraystretch{1.2}% 行距
\scriptsize
\centering
%cell大小
% \setlength{\aboverulesep}{1.85mm}
% \setlength{\belowrulesep}{-0.05mm}
\setlength{\tabcolsep}{0.88mm}{
\begin{tabular}{cc|cccccccccc}
\hline
\multicolumn{2}{c|}{} &\multicolumn{10}{c}{Major Body}\\
% \hline
\multicolumn{2}{c|}{Time (sec)}     & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8  & 0.9 & 1.0        \\
\hline
& LTD (D)~\cite{mao2019learning}
&4.3 &8.7 &12.7 &18.9 &24.5 &29.4 &34.0 &39.2 &43.4 &48.7\\

% & DMGNN (D)~\cite{li2020dynamic}  

% &23.0  &55.7  &107.7  &131.4
% \\
% &{PGBIG (D)~\cite{ma2022progressively}} 

% &22.6  &53.6  &104.3  &129.6
% \\

% 右手的结果需要更新
\multirow{-4}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{}}}
& {SPGSN (D)~\cite{li2022skeleton}}

&4.2 &9.3 &15.1 &21.0 &27.0 &32.6 &38.0 &43.2 &48.2 &52.6
\\

\hline
\hline
% RH 结果有点问题，需要重新训练
{\cellcolor{white}} & {\cellcolor{white}LTD (U)~\cite{mao2019learning}}

&4.1 &9.1 &14.4 &19.9&25.4 &30.5 &35.6 &40.6&45.5 &50.2\\

% & DMGNN (D)~\cite{li2020dynamic}  

% &23.0  &55.7  &107.7  &131.4
% \\
% &{PGBIG (D)~\cite{ma2022progressively}} 

% &22.6  &53.6  &104.3  &129.6
% \\

{\cellcolor{white}} & {SPGSN (U)~\cite{li2022skeleton}}   

&6.3 &12.7 &18.9 &24.5 &30.0 &34.9 &39.6 &44.4 &48.8 &53.4


\\
\hline
\hline

\multirow{-7}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{}}}

& {\cellcolor{white}\textbf{EAI} (Ours)}

&\textbf{3.9} &\textbf{8.3} &\textbf{13.4} &\textbf{18.7}&\textbf{23.9} &\textbf{28.8} &\textbf{33.7} &\textbf{38.4}&\textbf{42.6} &\textbf{46.8}
\\
\bottomrule

\end{tabular}
}
% \vspace{-.5em}
\end{table}

==> supmat/table_s_moreaction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t!]
\caption{\textbf{Detailed results on other action split} with the evaluation metrics MPJPE (in $mm$). (U) is the abbreviation of united training strategy. The best results are highlighted in bold.
}
\vspace{-.5em}
\renewcommand\arraystretch{1.4}%行距
\label{tab:s_moreaction}
\centering
\scriptsize
\setlength{\tabcolsep}{0.64mm}{
\begin{tabular}{cc|cccc|cccc|cccc|cccc|cccc|cccc}
\hline
\multicolumn{2}{c|}{Time (sec)} 
& 0.2 & 0.4 & 0.8 & 1.0 
& 0.2 & 0.4 & 0.8 & 1.0 
& 0.2 & 0.4 & 0.8 & 1.0 
& 0.2 & 0.4 & 0.8 & 1.0 
& 0.2 & 0.4 & 0.8 & 1.0 
& 0.2 & 0.4 & 0.8 & 1.0 
\\
\hline
\multicolumn{2}{c|}{Action} 
& \multicolumn{4}{c|}{ fly } 
& \multicolumn{4}{c|}{ see } 
& \multicolumn{4}{c|}{ peel } 
& \multicolumn{4}{c|}{ browse } 
& \multicolumn{4}{c|}{ takepicture } 
& \multicolumn{4}{c}{ inspect }  \\
{} & {LTD (U)~\cite{mao2019learning}}
 &29.1 &78.4 &170.0 &\textbf{181.7}
   &14.8 &43.0 &119.5 &153.6
   &27.3 &62.6 &111.1 &112.0
   &9.9 &23.2 &90.6 &133.4
   &\textbf{11.2} &\textbf{28.7} &115.0 &181.4
   &23.4 &59.2 &110.5 &120.6
\\
% {} & {DMGNN (U)~\cite{li2020dynamic}}
 
% \\
% {\cellcolor{white}} &{\cellcolor{white}PGBIG (U)~\cite{ma2022progressively}} 

% \\
{\cellcolor{white}} & {\cellcolor{white}SPGSN (U)~\cite{li2022skeleton}} 
&38.3 &88.6 &176.4 &211.2
   &20.3 &54.1 &124.7 &\textbf{140.7}
   &27.3 &\textbf{55.6} &\textbf{102.7} &\textbf{107.8}
   &11.7 &29.1 &54.0 &65.6
   &14.6 &33.3 &\textbf{108.3} &\textbf{165.2}
   &23.5 &56.9 &107.6 &121.7
\\
\multirow{-4}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{Whole body}}}
{\cellcolor{white}} &{\cellcolor{white} \textbf{EAI} (Ours)}
   &\textbf{26.1} &\textbf{70.7} &\textbf{160.0} &{188.1}
   &\textbf{14.2} &\textbf{42.5} &\textbf{114.3} &{143.9}
   &\textbf{24.8} &{59.3} &{113.4} &{118.6}
   &\textbf{7.3} &\textbf{18.8} &\textbf{38.3} &\textbf{49.1}
   &{11.8} &{33.4} &{112.1} &{165.5}
   &\textbf{21.2} &\textbf{55.3} &\textbf{106.8} &\textbf{115.7}
\\
\hline
\hline

%%%%%%%%%%%%. main body %%%%%%%%%%%%%%%%%%%%
\multicolumn{2}{c|}{Action} 
& \multicolumn{4}{c|}{ pour } 
& \multicolumn{4}{c|}{ use } 
& \multicolumn{4}{c|}{ wear } 
& \multicolumn{4}{c|}{ play } 
& \multicolumn{4}{c|}{ cook } 
& \multicolumn{4}{c}{ shake }  \\
{\cellcolor{white}} & {\cellcolor{white}LTD (U)~\cite{mao2019learning}}
&\textbf{23.1} &54.9 &83.3 &92.4
   &22.4 &57.5 &155.6 &185.9
   &\textbf{11.8} &\textbf{31.1} &87.9 &112.3
   &14.7 &39.3 &73.3 &92.2
   &25.7 &56.7 &86.3 &110.4
   &21.1 &\textbf{29.3} &\textbf{44.9} &52.0
\\
% {\cellcolor{white}} & {\cellcolor{white}DMGNN (U)~\cite{li2020dynamic}} 
  
% \\
% {\cellcolor{white}} &{\cellcolor{white}PGBIG (U)~\cite{ma2022progressively}} 

% \\
{\cellcolor{white}} & {\cellcolor{white}SPGSN (U)~\cite{li2022skeleton}} 
&27.1 &60.1 &85.6 &94.4
   &23.8 &59.1 &169.5 &207.4
   &13.7 &36.8 &89.5 &112.2
   &17.2 &40.3 &74.8 &90.6
   &29.8 &61.7 &\textbf{75.1} &\textbf{91.7}
   &28.5 &42.9 &72.4 &78.4
\\
\multirow{-4}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{Whole body}}}
{\cellcolor{white}} &{\cellcolor{white} \textbf{EAI} (Ours)}
&{24.6} &\textbf{53.7} &\textbf{79.0} &\textbf{81.4}
   &\textbf{19.4} &\textbf{51.6} &\textbf{145.5} &\textbf{178.1}
   &{13.9} &{35.6} &\textbf{76.7} &\textbf{96.1}
   &\textbf{12.0} &\textbf{32.6} &\textbf{68.2} &\textbf{86.4}
   &\textbf{23.7} &\textbf{50.1} &{76.8} &{100.3}
   &\textbf{18.3} &{33.9} &{45.1} &\textbf{49.5}
\\
\hline
\hline

%%%%%%%%%%%%. left hand %%%%%%%%%%%%%%%%%%%%
\multicolumn{2}{c|}{Action} 
& \multicolumn{4}{c|}{ chop } 
& \multicolumn{4}{c|}{ screw } 
& \multicolumn{4}{c|}{ toast } 
& \multicolumn{4}{c|}{ call } 
& \multicolumn{4}{c|}{ stamp } 
& \multicolumn{4}{c}{ staple }  \\
{\cellcolor{white}} & {\cellcolor{white}LTD (U)~\cite{mao2019learning}}
&\textbf{16.5} &\textbf{36.1} &67.7 &82.9
   &14.9 &31.5 &149.7 &214.6
   &16.7 &41.5 &\textbf{78.8} &117.1
   &\textbf{12.3} &33.1 &\textbf{83.7} &\textbf{100.2}
   &\textbf{12.8} &\textbf{22.7} &66.0 &124.2
   &\textbf{14.2} &\textbf{24.5} &\textbf{60.2} &91.1
\\
% {\cellcolor{white}} & {\cellcolor{white}DMGNN (U)~\cite{li2020dynamic}} 
 
% \\
% {\cellcolor{white}} &{\cellcolor{white}PGBIG(U)~\cite{ma2022progressively}}

% \\
{\cellcolor{white}} & {\cellcolor{white}SPGSN (U)~\cite{li2022skeleton}} 
   &20.2 &38.2 &\textbf{62.1} &\textbf{77.7}
   &13.8 &\textbf{30.2} &141.8 &200.7
   &17.7 &\textbf{41.0} &79.6 &121.5
   &12.6 &\textbf{32.1} &86.3 &107.1
   &16.0 &25.6 &\textbf{59.7} &\textbf{101.3}
   &18.8 &32.7 &62.6 &\textbf{90.9}
\\
\multirow{-4}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{Whole body}}}
{\cellcolor{white}} &{\cellcolor{white} \textbf{EAI} (Ours)}
&{18.4} &{37.9} &{67.0} &{79.9}
   &\textbf{13.4} &{31.5} &\textbf{113.7} &\textbf{135.0}
   &\textbf{15.5} &{41.2} &{91.1} &\textbf{104.8}
   &{12.7} &{38.4} &{91.4} &{111.4}
   &{14.2} &{27.2} &{77.5} &{126.2}
   &{14.9} &{30.0} &{67.9} &{95.2}
\\
\hline
\hline

\hline
\end{tabular}}
\vspace{-.7em}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> supmat/table_s_righthand.tex <==
% SPGSN (AW)的结果和Wholebody的结果都需要更新，正在跑

% 30 没有A（w/o MMD loss; w/o DN）
% 31 # 没有A（w MMD loss; w/o DN）
% 32 没有A（w/0 MMD loss; w DN）
% 33  没有I（w/0 Phy; w/0 S）
% 34  没有I（w/0 Phy; w S）
% 35  没有I（w Phy; w/o S）

% 30 没有A,没有I（w/o MMD loss; w/o DN）
% 
%  \textbf{(3)} As to the key components of our method, we can observe that XCI is the most important design. With the help of XCA, the extracted interaction information is more expressive and lead to more high-fidelity prediction.

\begin{table}[t]
% \vspace{-1.5em}
\caption{{Average results of right hand with finer intervals.} }
\label{tab:s_rh}
\vspace{-.7em}
\renewcommand\arraystretch{1.3}% 行距
\scriptsize
\centering
%cell大小
% \setlength{\aboverulesep}{1.85mm}
% \setlength{\belowrulesep}{-0.05mm}
\setlength{\tabcolsep}{0.6mm}{
\begin{tabular}{cc|cccccccccc}
\hline
 \multicolumn{2}{c|}{} &\multicolumn{10}{c}{Right Hand}\\
% \hline
\multicolumn{2}{c|}{Time (sec)}     & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8  & 0.9 & 1.0        \\
\hline
& LTD (D)~\cite{mao2019learning}

&12.8 &34.3 &55.1 &75.5 &101.2 &122.6 &141.0 &153.0 &176.7 &190.8\\



% 右手的结果需要更新
\multirow{-4}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{}}}
& {SPGSN (D)~\cite{li2022skeleton}}

&14.7 &37.2 &60.0 &81.5 &104.3 &127.1 &147.1 &165.9 &184.4 &202.8
\\

\hline
\hline
% RH 结果有点问题，需要重新训练
{\cellcolor{white}} & {\cellcolor{white}LTD (U)~\cite{mao2019learning}}

&12.2 &32.3 &53.2 &74.6&96.4 &116.4 &136.8 &157.8&177.2 &195.5\\
% &Res. sup.~\cite{martinez2017human}& \\

{\cellcolor{white}} & {SPGSN (U)~\cite{li2022skeleton}}   

&13.5 &34.3 &56.1 &75.5 &98.2 &118.2 &135.9 &153.0 &170.6 &190.8

\\


\hline
\hline

\multirow{-7}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{}}}


& {\cellcolor{white}\textbf{EAI} (Ours)}

&\textbf{11.1} &\textbf{29.8} &\textbf{49.4} &\textbf{69.0}&\textbf{88.0} &\textbf{106.1} &\textbf{124.0} &\textbf{140.6}&\textbf{154.3} &\textbf{169.0}
\\
\bottomrule

\end{tabular}
}
\vspace{-1.5em}
\end{table}

==> supmat/table_s_suba.tex <==
\begin{table*}[!ht]
\scriptsize
\renewcommand\arraystretch{1.2}% 行距
\centering
\caption{145 sub-action types of S10. }
\vspace{-.5em}
\setlength{\tabcolsep}{4.5mm}{
\begin{tabular}{|lllll|}
\hline
\multicolumn{1}{|l|}{airplane-fly-1}       & \multicolumn{1}{l|}{cubemedium-lift-1}        & \multicolumn{1}{l|}{fryingpan-cook-2}      & \multicolumn{1}{l|}{phone-call-1}            & stapler-staple-2      \\ \hline
\multicolumn{1}{|l|}{airplane-lift-1}      & \multicolumn{1}{l|}{cubemedium-pass-1}        & \multicolumn{1}{l|}{gamecontroller-lift-1} & \multicolumn{1}{l|}{phone-lift-1}            & teapot-pass-1         \\ \hline
\multicolumn{1}{|l|}{airplane-pass-1}      & \multicolumn{1}{l|}{cubesmall-inspect-1}      & \multicolumn{1}{l|}{gamecontroller-pass-1} & \multicolumn{1}{l|}{phone-pass-1}            & teapot-pour-1         \\ \hline
\multicolumn{1}{|l|}{alarmclock-lift-1}    & \multicolumn{1}{l|}{cubesmall-lift-1}         & \multicolumn{1}{l|}{gamecontroller-play-1} & \multicolumn{1}{l|}{piggybank-pass-1}        & teapot-pour-2         \\ \hline
\multicolumn{1}{|l|}{alarmclock-pass-1}    & \multicolumn{1}{l|}{cubesmall-pass-1}         & \multicolumn{1}{l|}{hammer-lift-1}         & \multicolumn{1}{l|}{piggybank-use-1}         & toothpaste-lift-1     \\ \hline
\multicolumn{1}{|l|}{alarmclock-see-1}     & \multicolumn{1}{l|}{cup-drink-1}              & \multicolumn{1}{l|}{hammer-pass-1}         & \multicolumn{1}{l|}{pyramidlarge-pass-1}     & toothpaste-pass-1     \\ \hline
\multicolumn{1}{|l|}{apple-eat-1}          & \multicolumn{1}{l|}{cup-drink-2}              & \multicolumn{1}{l|}{hammer-use-1}          & \multicolumn{1}{l|}{pyramidmedium-inspect-1} & toothpaste-squeeze-1  \\ \hline
\multicolumn{1}{|l|}{apple-pass-1}         & \multicolumn{1}{l|}{cup-lift-1}               & \multicolumn{1}{l|}{hammer-use-2}          & \multicolumn{1}{l|}{pyramidmedium-lift-1}    & toothpaste-squeeze-2  \\ \hline
\multicolumn{1}{|l|}{banana-eat-1}         & \multicolumn{1}{l|}{cup-pass-1}               & \multicolumn{1}{l|}{hammer-use-3}          & \multicolumn{1}{l|}{pyramidmedium-pass-1}    & toruslarge-inspect-1  \\ \hline
\multicolumn{1}{|l|}{banana-lift-1}        & \multicolumn{1}{l|}{cup-pour-1}               & \multicolumn{1}{l|}{hand-inspect-1}        & \multicolumn{1}{l|}{pyramidsmall-inspect-1}  & toruslarge-lift-1     \\ \hline
\multicolumn{1}{|l|}{banana-pass-1}        & \multicolumn{1}{l|}{cylinderlarge-inspect-1}  & \multicolumn{1}{l|}{hand-lift-1}           & \multicolumn{1}{l|}{scissors-pass-1}         & toruslarge-pass-1     \\ \hline
\multicolumn{1}{|l|}{banana-peel-1}        & \multicolumn{1}{l|}{cylinderlarge-lift-1}     & \multicolumn{1}{l|}{hand-pass-1}           & \multicolumn{1}{l|}{scissors-use-1}          & torusmedium-inspect-1 \\ \hline
\multicolumn{1}{|l|}{banana-peel-2}        & \multicolumn{1}{l|}{cylinderlarge-pass-1}     & \multicolumn{1}{l|}{hand-shake-1}          & \multicolumn{1}{l|}{spherelarge-inspect-1}   & torusmedium-lift-1    \\ \hline
\multicolumn{1}{|l|}{binoculars-lift-1}    & \multicolumn{1}{l|}{cylindermedium-inspect-1} & \multicolumn{1}{l|}{headphones-lift-1}     & \multicolumn{1}{l|}{spherelarge-lift-1}      & torusmedium-pass-1    \\ \hline
\multicolumn{1}{|l|}{binoculars-pass-1}    & \multicolumn{1}{l|}{cylindermedium-pass-1}    & \multicolumn{1}{l|}{headphones-pass-1}     & \multicolumn{1}{l|}{spherelarge-pass-1}      & torussmall-inspect-1  \\ \hline
\multicolumn{1}{|l|}{binoculars-see-1}     & \multicolumn{1}{l|}{cylindersmall-inspect-1}  & \multicolumn{1}{l|}{headphones-use-1}      & \multicolumn{1}{l|}{spheremedium-inspect-1}  & torussmall-lift-1     \\ \hline
\multicolumn{1}{|l|}{bowl-drink-1}         & \multicolumn{1}{l|}{cylindersmall-pass-1}     & \multicolumn{1}{l|}{knife-chop-1}          & \multicolumn{1}{l|}{spheremedium-lift-1}     & torussmall-pass-1     \\ \hline
\multicolumn{1}{|l|}{bowl-drink-2}         & \multicolumn{1}{l|}{doorknob-lift-1}          & \multicolumn{1}{l|}{knife-pass-1}          & \multicolumn{1}{l|}{spheremedium-pass-1}     & train-lift-1          \\ \hline
\multicolumn{1}{|l|}{bowl-lift-1}          & \multicolumn{1}{l|}{doorknob-use-1}           & \multicolumn{1}{l|}{knife-peel-1}          & \multicolumn{1}{l|}{spheresmall-inspect-1}   & train-pass-1          \\ \hline
\multicolumn{1}{|l|}{bowl-pass-1}          & \multicolumn{1}{l|}{doorknob-use-2}           & \multicolumn{1}{l|}{lightbulb-pass-1}      & \multicolumn{1}{l|}{spheresmall-pass-1}      & train-play-1          \\ \hline
\multicolumn{1}{|l|}{camera-browse-1}      & \multicolumn{1}{l|}{duck-pass-1}              & \multicolumn{1}{l|}{lightbulb-screw-1}     & \multicolumn{1}{l|}{stamp-lift-1}            & watch-pass-1          \\ \hline
\multicolumn{1}{|l|}{camera-pass-1}        & \multicolumn{1}{l|}{elephant-inspect-1}       & \multicolumn{1}{l|}{mouse-lift-1}          & \multicolumn{1}{l|}{stamp-pass-1}            & waterbottle-drink-1   \\ \hline
\multicolumn{1}{|l|}{camera-takepicture-1} & \multicolumn{1}{l|}{elephant-pass-1}          & \multicolumn{1}{l|}{mouse-pass-1}          & \multicolumn{1}{l|}{stamp-stamp-1}           & waterbottle-pass-1    \\ \hline
\multicolumn{1}{|l|}{camera-takepicture-2} & \multicolumn{1}{l|}{eyeglasses-wear-1}        & \multicolumn{1}{l|}{mouse-use-1}           & \multicolumn{1}{l|}{stanfordbunny-inspect-1} & waterbottle-pour-1    \\ \hline
\multicolumn{1}{|l|}{camera-takepicture-3} & \multicolumn{1}{l|}{flashlight-on-1}          & \multicolumn{1}{l|}{mug-drink-1}           & \multicolumn{1}{l|}{stanfordbunny-lift-1}    & wineglass-drink-1     \\ \hline
\multicolumn{1}{|l|}{cubelarge-inspect-1}  & \multicolumn{1}{l|}{flashlight-on-2}          & \multicolumn{1}{l|}{mug-drink-2}           & \multicolumn{1}{l|}{stanfordbunny-pass-1}    & wineglass-drink-2     \\ \hline
\multicolumn{1}{|l|}{cubelarge-lift-1}     & \multicolumn{1}{l|}{flute-pass-1}             & \multicolumn{1}{l|}{mug-lift-1}            & \multicolumn{1}{l|}{stapler-lift-1}          & wineglass-lift-1      \\ \hline
\multicolumn{1}{|l|}{cubelarge-pass-1}     & \multicolumn{1}{l|}{flute-play-1}             & \multicolumn{1}{l|}{mug-pass-1}            & \multicolumn{1}{l|}{stapler-pass-1}          & wineglass-pass-1      \\ \hline
\multicolumn{1}{|l|}{cubemedium-inspect-1} & \multicolumn{1}{l|}{fryingpan-cook-1}         & \multicolumn{1}{l|}{mug-toast-1}           & \multicolumn{1}{l|}{stapler-staple-1}        & wineglass-toast-1     \\ \hline
\end{tabular}
}
\label{Table:subaction}
\end{table*}


==> supmat/table_s_united.tex <==
% SPGSN (AW)的结果和Wholebody的结果都需要更新，正在跑

% 30 没有A（w/o MMD loss; w/o DN）
% 31 # 没有A（w MMD loss; w/o DN）
% 32 没有A（w/0 MMD loss; w DN）
% 33  没有I（w/0 Phy; w/0 S）
% 34  没有I（w/0 Phy; w S）
% 35  没有I（w Phy; w/o S）

% 30 没有A,没有I（w/o MMD loss; w/o DN）
% 
%  \textbf{(3)} As to the key components of our method, we can observe that XCI is the most important design. With the help of XCA, the extracted interaction information is more expressive and lead to more high-fidelity prediction.

\begin{table}[h]
% \vspace{-1.5em}
\caption{{Average results on all actions with finer intervals.} }
\label{tab:s_wb}
\vspace{-.5em}
\renewcommand\arraystretch{1.2}% 行距
\scriptsize
\centering
%cell大小
% \setlength{\aboverulesep}{1.85mm}
% \setlength{\belowrulesep}{-0.05mm}
\setlength{\tabcolsep}{0.72mm}{
\begin{tabular}{cc|cccccccccc}
\hline
 \multicolumn{2}{c|}{} &\multicolumn{10}{c}{Whole Body}\\
% \hline
\multicolumn{2}{c|}{Time (sec)}     & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8  & 0.9 & 1.0        \\
\hline
& LTD (D)~\cite{mao2019learning}

&7.5 &18.4 &30.9 &45.3&60.0 &73.9 &87.0 &100.3&112.4 &125.0\\
% & DMGNN (D)~\cite{li2020dynamic}  

% &23.0  &55.7  &107.7  &131.4
% \\
% &{PGBIG (D)~\cite{ma2022progressively}} 

% &22.6  &53.6  &104.3  &129.6
% \\
% 右手的结果需要更新
\multirow{-4}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{}}}
& {SPGSN (D)~\cite{li2022skeleton}}

&8.7 &21.2 &34.9 &48.4&62.0 &75.3 &87.9 &100.3&112.4 &124.0\\

\hline
\hline
% RH 结果有点问题，需要重新训练
{\cellcolor{white}} & {\cellcolor{white}LTD (U)~\cite{mao2019learning}}

&7.4 &18.4 &30.5 &43.1&55.9 &68.5 &81.6 &95.2&108.2 &120.4\\
% &Res. sup.~\cite{martinez2017human}& \\
% {\cellcolor{white}} & DMGNN (U)~\cite{li2020dynamic}  

% &22.7  &50.0 &98.9  &128.2
% \\
% {\cellcolor{white}} &{PGBIG (U)~\cite{ma2022progressively}} 

% &22.2  &48.1  &97.4  &125.8
% \\
{\cellcolor{white}} & {SPGSN (U)~\cite{li2022skeleton}}   

&8.9 &21.0 &34.3 &46.9 &60.3 &72.6 &84.5 &96.3 &107.7 &120.3



\\
\hline
\hline

\multirow{-7}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{}}}


& {\cellcolor{white}\textbf{EAI} (Ours)}

&\textbf{6.4} &\textbf{16.7} &\textbf{28.6} &\textbf{40.7}&\textbf{52.5} &\textbf{63.7} &\textbf{75.0} &\textbf{85.8}&\textbf{95.2} &\textbf{104.6}
\\
\bottomrule

\end{tabular}
}
\vspace{-.5em}
\end{table}

 

==> tabletex/pseudocode.tex <==
\begin{table}[]
\centering
\caption{Path Planning algorithm pseudocode.}
\scalebox{0.9}{
\begin{tabular}{cccc}
\toprule
Models  & Seen tasks & Unseen Objects & Backgrounds \\ \midrule
QUART1 &            &                &             \\ 
QUART2 &            &                &             \\ 
xxx    &            &                &             \\ \bottomrule
\end{tabular}}
\end{table}

==> tabletex/tab1_cc.tex <==
\begin{table}[]
\centering
\caption{ xxxxx.}
\scalebox{0.9}{
\begin{tabular}{cccc}
\toprule
Models  & Seen tasks & Unseen Objects & Backgrounds \\ \midrule
QUART1 &            &                &             \\ 
QUART2 &            &                &             \\ 
xxx    &            &                &             \\ \bottomrule
\end{tabular}}
\end{table}

==> tabletex/tab2_cc.tex <==
\begin{table}[htp]
\centering
\caption{ xxxxx.}
\scalebox{0.9}{
\begin{tabular}{ccccc}
\toprule
       &     & \multicolumn{3}{c}{Generalization Scenario Levels} \\ \cmidrule{3-5}
Models  & All & \makebox[0.1\textwidth][c]{L1}              & \makebox[0.1\textwidth][c]{L2}              & \makebox[0.1\textwidth][c]{L3}             \\ \midrule
QUART1 &     &                 &                 &                \\
QUART2 &     &                 &                 &                \\
xxx    &     &                 &                 &                \\ \bottomrule
\end{tabular}}
\end{table}

==> tabletex/tab3_cc.tex <==
\begin{table}[t]
\centering
\caption{ xxxxx.}
\scalebox{0.9}{
\begin{tabular}{ccccc}
\toprule
       &       & Real Objects                                                   & \multicolumn{2}{c}{SimObjects(not seen in real)}                                                                                  \\ \cmidrule(r){3-3} \cmidrule(r){4-5} 
Models  & Ratio & \begin{tabular}[c]{@{}c@{}}Seen Skill\\ w/Objects\end{tabular} & \begin{tabular}[c]{@{}c@{}}Seen Skill\\ w/Objects\end{tabular} & \begin{tabular}[c]{@{}c@{}}Unseen Skill\\ w/Objects\end{tabular} \\ \midrule
QUART1 & 1/8   &                                                                &                                                                &                                                                  \\
QUART1 & 1/64   &                                                                &                                                                &                                                                  \\
QUART1 & 1/1   &                                                                &                                                                &                                                                  \\
QUART2 & 0.8   &                                                                &                                                                &                                                                  \\
xxx    &       &                                                                &                                                                &                                                                  \\ \bottomrule
\end{tabular}}
\end{table}

==> tabletex/tab4_cc.tex <==
\begin{table*}[ht]
\scriptsize
\centering
\caption{ \zhao{the results has not to be added.}}
\label{table:holdouttasks}
\begin{center}
\begin{tabular}{p{1.2cm} p{4cm} p{1.8cm} p{1.8cm} p{1.8cm} p{1.8cm}}
\toprule
       &     & \multicolumn{2}{c}{\textbf{QUART1}} & \multicolumn{2}{c}{\textbf{QUART2}} \\ \cmidrule(r){3-4} \cmidrule(r){5-6}
\textbf{Skill} &\textbf{Tasks(Seen/Unseen)} &
\textbf{Sim} & \textbf{Real} & \textbf{Sim} & \textbf{Real}\\
\midrule
\multirow{3}{*}{unload} &`unload orange traybox' & 0\% (0) & 10\% (6.7) & 0\% (0) \\
&`unload red traybox' & 20\% (12.7) & 0\% (0) & 0\% (0) \\
&`unload gold traybox' & 10\% (9.49) & 0\% (0) & 0\% (0) \\
\arrayrulecolor{black!30}\cmidrule{2-6}
\multirow{3}{*}{unload} &`unload orange traybox' & 0\% (0) & 10\% (6.7) & 0\% (0) \\
&`unload red traybox' & 20\% (12.7) & 0\% (0) & 0\% (0) \\
&`unload gold traybox' & 10\% (9.49) & 0\% (0) & 0\% (0) \\
\arrayrulecolor{black!30}\cmidrule{2-6}
\multirow{3}{*}{unload} &`unload orange traybox' & 0\% (0) & 10\% (6.7) & 0\% (0) \\
&`unload red traybox' & 20\% (12.7) & 0\% (0) & 0\% (0) \\
&`unload gold traybox' & 10\% (9.49) & 0\% (0) & 0\% (0) \\

\arrayrulecolor{black}\midrule
\multirow{3}{*}{go avoid} &`go avoid texture oven' & 50\% (15.8) & 75\% (9.7) & 7.5\% (4.2) \\
&`go avoid texture table' & 50\% (15.8)& 75\% (9.7) & 0\% (0) \\
&`go avoid texture trashcan' & 70\% (14.5) & 70\% (10.3) & 0\% (0) \\
% &`place bottle in table surface' & 0 & 50\% (11.2) & 5\% (3.5) \\
% &`place white sponge in purple bowl' & 70\% (14.9)& 45\% (11.2) & 0\% (0) \\
% &`place white sponge in tray' & 50\% (15.8) & 40\% (11.0) & 0\% (0) \\
% &`place apple in ceramic bowl' & 30\% (14.5) & 20\% (8.9) & 0\% (0) \\
% &`place bottle in purple bowl' & 30\% (14.5) & 20\% (8.9) & 0\% (0) \\
% %`place plastic cup in the ceramic bowl' & 0\% (0) & N/A \\
% &`place banana in ceramic cup' & 10\% (9.5) & 0\% (0) & 0\% (0) \\
% &`place banana on white sponge' & 40\% (15.5) & 0\% (0) & 0\% (0) \\
% &`place metal cup in red bowl' & 0\% (0) & 0\% (0) & 0\% (0) \\
\arrayrulecolor{black!30}\cmidrule{2-6}
\multirow{3}{*}{crawl} &`pick up grapes' & 70\% (14.5) & 65\% (10.7) & 0\% (0) \\
&`pick up apple' & 20\% (12.7) & 55\% (11.2) & 5\% (3.5) \\
&`pick up towel' & 50\% (15.8) & 42.8\% (18.7) & 0\% (0) \\
% &`pick up pepper' & 50\% (15.8)  & 35\% (10.7) & 12.5\% (5.2) \\
% &`pick up bottle' & 40\% (15.5) & 30\% (10.3)& 17.5\% (6.0) \\
% &`pick up the red bowl' & 30\% (14.5) & 0\% (0) & 0\% (0) \\
\arrayrulecolor{black!30}\cmidrule{2-6}
\multirow{3}{*}{go through } &`crawl red bar1' & 0\% (0) & 14\% (13.2) & 0\% (0) \\
&`crawl red bar2' & 0\% (0) & 14\% (13.2) & 0\% (0) \\
&`crawl red bar3' & 0\% (0) & 14\% (13.2) & 0\% (0) \\
\arrayrulecolor{black!30}\cmidrule{2-6}
\multirow{3}{*}{unload} &`unload orange traybox' & 0\% (0) & 10\% (6.7) & 0\% (0) \\
&`unload red traybox' & 20\% (12.7) & 0\% (0) & 0\% (0) \\
&`unload gold traybox' & 10\% (9.49) & 0\% (0) & 0\% (0) \\
\arrayrulecolor{black!30}\cmidrule{2-6}
\multirow{3}{*}{distinguish} &`distinguish texture e' & 50\% (15.8) & 30\% (10.3) & 0\% (0) \\
&`distinguish texture d' & 30\% (14.5) & 25\% (9.7) & 0\% (0) \\
&`distinguish texture c' & 60\% (15.5) & 0\% (0) & 0\% (0) \\
\arrayrulecolor{black!30}\cmidrule{2-6}
\multirow{3}{*}{go to} &`go to texture table' & 50\% (15.8) & 30\% (10.3) & 0\% (0) \\
&`go to texture wardrobe' & 30\% (14.5) & 25\% (9.7) & 0\% (0) \\
&`go to texture vase' & 60\% (15.5) & 0\% (0) & 0\% (0) \\
\arrayrulecolor{black!30}\cmidrule{2-6}
\multirow{3}{*}{stop} &`stop cyan ball' & 50\% (15.8) & 30\% (10.3) & 0\% (0) \\
&`stop navy ball' & 30\% (14.5) & 25\% (9.7) & 0\% (0) \\
&`stop gray ball' & 60\% (15.5) & 0\% (0) & 0\% (0) \\
\arrayrulecolor{black}\midrule
&\textit{Holdout Task Overall} & 38\% & 32\% & 4\% \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-15pt}
\end{table*}



==> tabletex/table1_united.tex <==
% SPGSN (PAW)的结果和Wholebody的结果都需要更新，正在跑

% 30 没有A（w/o MMD loss; w/o DN）
% 31 # 没有A（w MMD loss; w/o DN）
% 32 没有A（w/0 MMD loss; w DN）
% 33  没有I（w/0 Phy; w/0 S）
% 34  没有I（w/0 Phy; w S）
% 35  没有I（w Phy; w/o S）

% 30 没有A,没有I（w/o MMD loss; w/o DN）
% 
%  \textbf{(3)} As to the key components of our method, we can observe that XCI is the most important design. With the help of XCA, the extracted interaction information is more expressive and lead to more high-fidelity prediction.

\begin{table*}[t!]
 \vspace{-1.em}
\caption{\textbf{Average results on all actions} with the evaluation metrics  MPJPE and MPJPE-AW (in $mm$). (AW), (D) and (U) are the abbreviation of the MPJPE-AW, \textbf{divided} and \textbf{united} training strategies. A lower value means better performance. The best results are highlighted in bold. Notably, {EAI} is only trained with united training strategies due to the need to explore body components' interactions.
(1) Compared with other baselines using a divided strategy, which lacks the interaction of components, our EAI outperforms them on all actions. It indicates the necessity of cross-context interaction. (2) Regarding the united strategy, which does not consider the heterogeneity of different body parts, our results are superior to other methods, which reveals the effectiveness of our cross-context alignment.}
\label{tab:united}
\vspace{-1em}
\renewcommand\arraystretch{1.1}% 行距
\scriptsize
\centering
%cell大小
% \setlength{\aboverulesep}{1.85mm}
% \setlength{\belowrulesep}{-0.05mm}
\setlength{\tabcolsep}{0.83mm}{
\begin{tabular}{cc|cccc|cccc|cccc|cccc|cccc|cccc}
\hline
\multicolumn{2}{c|}{Body Parts} &\multicolumn{4}{c|}{Major body} &\multicolumn{4}{c|}{Left Hands} & \multicolumn{4}{c|}{Right Hands} &\multicolumn{4}{c|}{Left Hands (AW)} &\multicolumn{4}{c|}{Right Hands (AW)} &\multicolumn{4}{c}{Whole Body}\\
% \hline
\multicolumn{2}{c|}{Time (sec)} & 0.2 & 0.4 & 0.8 & 1.0    & 0.2 & 0.4 & 0.8 & 1.0    & 0.2 & 0.4 & 0.8 & 1.0   & 0.2 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0   & 0.2 & 0.4 & 0.8 & 1.0       \\
\hline
& LTD (D)~\cite{mao2019learning}
&8.7  &18.9 &39.2  &48.7
&19.7 &57.0 &143.3 &181.5
&33.3 &77.5 &159.1 &195.6
&9.1  &18.3 &33.8  &41.4
&17.2 &28.3 &46.1  &53.1
&18.3 &45.6 &101.5 &126.1
\\
& DMGNN (D)~\cite{li2020dynamic}  
&11.2  &23.1  &43.8   &53.5     
&24.8  &62.0  &153.2  &190.1    
&38.1  &83.0  &166.7  &205.7 
&10.0  &21.7  &39.1   &44.4
&21.6  &32.6  &49.7   &60.5
&23.0  &55.7  &107.7  &131.4
\\
&{PGBIG (D)~\cite{ma2022progressively}} 
&10.4  &21.7  &44.0   &52.8     
&22.8  &61.5  &149.9  &186.7    
&37.6  &82.4  &164.5  &203.9    
&10.5  &22.2  &38.7   &43.5
&21.5  &31.1  &48.8   &58.7
&22.6  &53.6  &104.3  &129.6
\\
% 右手的结果需要更新
\multirow{-4}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{Divided}}}
& {SPGSN (D)~\cite{li2022skeleton}}
&9.3  &21.0 &43.2  &52.6 
&25.3 &61.1 &129.8 &164.2
&37.2 &81.5 &165.9 &202.8
&9.3  &18.5 &34.0  &41.6 
&16.1 &28.8 &49.3  &56.9
&21.2 &48.4 &100.3 &124.0
\\

\hline
\hline
% RH 结果有点问题，需要重新训练
{\cellcolor{white}} & {\cellcolor{white}LTD (U)~\cite{mao2019learning}}
&9.1 &19.9 &40.6 &50.2
&19.9 &50.5 &123.4 &162.5
&32.3 &74.6 &157.8 &195.5
&8.9 &17.1 &34.0 &42.5
&16.7 &29.3 &49.8 &58.3
&18.4 &43.1 &95.2 &120.4
\\
% &Res. sup.~\cite{martinez2017human}& \\
{\cellcolor{white}} & DMGNN (U)~\cite{li2020dynamic}  
&13.7  &26.4  &47.2  &56.9     
&22.4  &57.3  &141.1  &172.0    
&36.3  &78.9  &160.6  &203.7 
&9.7  &20.3  &38.2  &46.4
&19.0  &33.2  &52.6  &64.1
&22.7  &50.0 &98.9  &128.2
\\
{\cellcolor{white}} &{PGBIG (U)~\cite{ma2022progressively}} 
&13.2  &24.9  &45.0  &54.2      
&23.0  &56.4  &130.4  &165.7     
&35.0  &77.2  &156.1  &199.4     
&10.2  &19.5  &37.4  & 45.7
&19.1  &32.5  &53.4  &62.0
&22.2  &48.1  &97.4  &125.8
\\
{\cellcolor{white}} & {SPGSN (U)~\cite{li2022skeleton}}   
&12.7 &24.5 &44.4 &53.4
&21.6 &55.5 &126.0 &161.6
&34.3 &75.5 &153.0 &190.8
&9.6 &18.2 &34.8 &42.3
&18.5 &31.0 &50.7 &58.2
&21.0 &46.9 &96.3 &120.3
\\
\hline
\hline

\multirow{-7}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{United}}}


& {\cellcolor{white}\textbf{EAI} (Ours)}
&\textbf{8.3} &\textbf{18.7} &\textbf{38.4} &\textbf{46.8}
&\textbf{17.7} &\textbf{49.2} &\textbf{110.1} &\textbf{136.4}
&\textbf{29.8} &\textbf{69.0} &\textbf{140.6} &\textbf{169.0}
&\textbf{8.6} &\textbf{17.3} &\textbf{32.8} &\textbf{38.8}
&\textbf{16.2} &\textbf{27.8} &\textbf{45.5} &\textbf{51.6}
&\textbf{16.7} &\textbf{40.7} &\textbf{85.8} &\textbf{104.6}
\\
\hline

\end{tabular}
}
\vspace{-1.em}
\end{table*}

% PA 
% & LTD (D)
% &1.0 &2.3 &4.4 &5.0 & 2.3 &5.0 &8.0 &9.2\\
% \multirow{-4}{*}{}
% & {SPGSN (D)}
% &1.0 &2.0&3.8 &4.2 & 2.2 &4.7 &7.5 &8.5\\
% \hline
%  & {LTD (U)}
% &1.1 &2.4&5.3 &6.0 & 2.3 &5.2&9.3 &10.6\\
% & {SPGSN (U)}   
%  &1.3 &2.4 &4.9 &5.5 &2.3 &5.1 &8.7 &9.6\\
% \hline
% & {\textbf{EAI} (Ours)}
% &\textbf{0.9} &\textbf{2.0}&\textbf{3.3} &\textbf{3.7}
% &\textbf{2.1} &\textbf{4.2}&\textbf{6.6} &\textbf{7.6}\\

==> tabletex/table2_wholebody.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t!]
% \vspace{-1em}
\caption{\textbf{Detailed results on common action split} with the evaluation metrics MPJPE (in $mm$). (U) is the abbreviation of united training strategy. The best results are highlighted in bold. We observe that for both fine- and coarse-grained motion patterns, our results consistently outperform the competitors. 
It evidences the compatibility of our proposed EAI framework for various activities.
}
\vspace{-1em}
\renewcommand\arraystretch{1.15}%行距
\label{tab:wholebody}
\centering
\scriptsize
\setlength{\tabcolsep}{0.64mm}{
\begin{tabular}{cc|cccc|cccc|cccc|cccc|cccc|cccc}
\hline
\multicolumn{2}{c|}{Action} 
& \multicolumn{4}{c|}{A1 pass } 
& \multicolumn{4}{c|}{A2 eat } 
& \multicolumn{4}{c|}{A3 drink } 
& \multicolumn{4}{c|}{A4 lift } 
& \multicolumn{4}{c|}{A5 on } 
& \multicolumn{4}{c}{A6 squeeze }  \\
\multicolumn{2}{c|}{Time (sec)} 
& 0.2 & 0.4 & 0.8 & 1.0 
& 0.2 & 0.4 & 0.8 & 1.0 
& 0.2 & 0.4 & 0.8 & 1.0 
& 0.2 & 0.4 & 0.8 & 1.0 
& 0.2 & 0.4 & 0.8 & 1.0 
& 0.2 & 0.4 & 0.8 & 1.0 
\\
\hline
{} & {LTD (U)~\cite{mao2019learning}}
&21.4 &46.1 &85.1 &114.0
&21.0 &48.7 &102.3 &139.4
&25.9 &66.7 &115.7 &114.5
&16.3 &49.5 &113.0 &132.1
&19.7 &42.8 &70.1  &79.5
&14.3 &28.5 &43.6  &52.6
\\
{} & {DMGNN (U)~\cite{li2020dynamic}}
&25.7  &54.8  &91.2  &109.5  
&29.4  &60.2  &129.0 &170.6
&30.0  &74.4  &138.3 &163.7  
&18.2  &54.3  &118.9 &144.3 
&22.5  &51.0  &79.8  &91.0  
&18.4  &36.6  &58.3  &62.3  
\\
{\cellcolor{white}} &{\cellcolor{white}PGBIG (U)~\cite{ma2022progressively}} 
&23.9  &53.6  &88.7   &94.3
&25.3  &58.3  &118.9  &169.3  
&28.2  &72.1  &131.5  &159.9 
&17.1  &51.6  &116.5  &136.4 
&21.4  &49.4  &76.3   &85.6
&17.4  &35.7  &54.2   &61.0 
\\
{\cellcolor{white}} & {\cellcolor{white}SPGSN (U)~\cite{li2022skeleton}} 
&23.6 &51.0 &72.8  &90.6
&27.0 &57.9 &125.7 &165.8
&27.2 &70.9 &136.2 &156.3
&16.2 &48.9 &112.3 &130.1
&21.3 &48.7 &74.9  &79.9
&16.6 &33.5 &50.2  &58.8
\\
\multirow{-5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{Whole body}}}
{\cellcolor{white}} &{\cellcolor{white} \textbf{EAI} (Ours)}

&\textbf{16.9} &\textbf{37.0} &\textbf{61.2} &\textbf{72.9}
&\textbf{18.3} &\textbf{44.5} &\textbf{88.8} &\textbf{122.7}
&\textbf{20.4} &\textbf{54.7} &\textbf{90.3} &\textbf{83.7}
&\textbf{11.6} &\textbf{34.5} &\textbf{78.9} &\textbf{92.9}
&\textbf{15.8} &\textbf{36.5} &\textbf{57.7} &\textbf{66.6}
&\textbf{11.7} &\textbf{27.1} &\textbf{37.8} &\textbf{46.2}
\\
\hline
\hline

%%%%%%%%%%%%. main body %%%%%%%%%%%%%%%%%%%%
{\cellcolor{white}} & {\cellcolor{white}LTD (U)~\cite{mao2019learning}}
&10.2 &20.8 &33.2 &42.4
&12.1 &28.0 &\textbf{56.2} &\textbf{71.7}
&12.2 &23.4 &37.6 &40.1
&7.9 &20.3 &45.4 &54.9
&9.8 &17.8 &31.4 &36.4
&5.6 &12.7 &22.2 &26.6
\\
{\cellcolor{white}} & {\cellcolor{white}DMGNN (U)~\cite{li2020dynamic}} 
&11.7  &26.4  &35.1  &40.7  
&17.9  &37.6  &68.9  &88.4  
&14.5  &32.1  &44.8  &58.0
&12.1  &26.3  &51.1  &61.5  
&12.2  &22.0  &36.8  &42.5  
&23.1  &48.1  &64.2  &75.4  
\\
{\cellcolor{white}} &{\cellcolor{white}PGBIG (U)~\cite{ma2022progressively}} 
&12.0  &26.9  &34.7  &38.9 
&17.5  &36.5  &66.4  &83.2  
&15.7  &30.2  &42.6  &53.2 
&11.4  &24.3  &48.9  & 62.4 
&13.0  &20.7  &34.9  &41.2 
&21.5  &46.2  &60.3  & 72.4 
\\
{\cellcolor{white}} & {\cellcolor{white}SPGSN (U)~\cite{li2022skeleton}} 
&13.1 &25.8 &31.5 &35.1
&18.4 &34.8 &65.1 &82.0
&15.6 &28.9 &40.0 &48.6
&10.6 &22.6 &44.0 &51.6
&12.4 &21.7 &34.8 &39.3
&7.9 &13.8 &23.6 &27.9
\\
\multirow{-5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{Major body}}}
{\cellcolor{white}} &{\cellcolor{white} \textbf{EAI} (Ours)}
% &\textbf{8.7} &\textbf{19.2} &\textbf{26.8} &\textbf{31.4}
% &\textbf{10.2} &\textbf{26.3} &\textbf{53.9} &\textbf{67.6}
% &\textbf{9.2} &\textbf{16.8} &\textbf{25.9} &\textbf{26.3}
% &\textbf{6.8} &\textbf{17.7} &\textbf{37.8} &\textbf{44.9}
% &\textbf{7.3} &\textbf{14.2} &\textbf{25.0} &\textbf{29.5}
% &\textbf{5.4} &\textbf{12.0} &\textbf{21.1} &\textbf{26.0}
   &\textbf{9.0} &\textbf{19.7} &\textbf{28.4} &\textbf{31.6}
   &\textbf{10.5} &\textbf{26.4} &{57.0} &{72.5}
   &\textbf{10.2} &\textbf{19.1} &\textbf{30.2} &\textbf{30.8}
   &\textbf{6.5} &\textbf{16.4} &\textbf{36.4} &\textbf{44.4}
   &\textbf{7.9} &\textbf{15.6} &\textbf{26.3} &\textbf{31.3}
   &\textbf{5.4} &\textbf{12.2} &\textbf{20.2} &\textbf{24.4}
\\
\hline
\hline

%%%%%%%%%%%%. left hand %%%%%%%%%%%%%%%%%%%%
{\cellcolor{white}} & {\cellcolor{white}LTD (U)~\cite{mao2019learning}}
&\textbf{24.4} &\textbf{52.2}  &141.8 &211.2
&21.7 &52.5  &129.4 &187.5
&51.8 &123.4 &189.9 &185.8
&21.0 &66.3  &145.7 &163.8
&12.1 &34.1  &43.3  &50.1
&18.1 &35.6  &41.9  &54.6
\\
{\cellcolor{white}} & {\cellcolor{white}DMGNN (U)~\cite{li2020dynamic}} 
&36.7  &68.9  &137.8  &196.6 
&38.6  &87.5  &178.3  &234.4  
&56.2  &128.8  &210.5  &265.4  
&22.2  &68.7  &152.5  &181.2  
&15.3  &44.3  &54.3  &54.2  
&24.1  &49.3  &60.2  &73.1 
\\
{\cellcolor{white}} &{\cellcolor{white}PGBIG(U)~\cite{ma2022progressively}}
&33.5  &66.3  &140.0  &186.2 
&36.9  &88.2  &156.2  & 225.6
&56.7  &126.4  &215.7  & 264.6
&23.1  &66.9  &154.0  & 178.4 
&15.0  &43.2  &53.1  & 50.1 
&23.0  &45.6  &56.7  & 72.4 
\\
{\cellcolor{white}} & {\cellcolor{white}SPGSN (U)~\cite{li2022skeleton}} 
&30.9 &71.1  &114.4 &165.1
&36.5 &94.6  &206.1 &263.6
&51.4 &119.8 &219.3 &242.7
&20.3 &65.2  &152.9 &175.5
&14.9 &41.1  &50.1  &53.7
&22.9 &47.3  &55.2  &70.3
\\
\multirow{-5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{Left hands}}}
{\cellcolor{white}} &{\cellcolor{white} \textbf{EAI} (Ours)}
% &\textbf{27.2} &\textbf{62.2} &\textbf{107.6} &\textbf{152.6}
% &\textbf{21.7} &\textbf{47.6} &\textbf{120.3} &\textbf{181.8}
% &\textbf{42.2} &\textbf{71.1} &\textbf{121.1} &\textbf{132.7}
% &\textbf{18.0} &\textbf{61.8} &\textbf{139.5} &\textbf{159.3}
% &\textbf{10.6} &\textbf{30.2} &\textbf{36.9}  &\textbf{43.8}
% &\textbf{13.9} &\textbf{29.7} &\textbf{34.5}  &\textbf{47.6}
   &{25.4} &{52.6} &\textbf{104.9} &\textbf{145.1}
   &\textbf{17.8} &\textbf{49.0} &\textbf{96.5} &\textbf{148.7}
   &\textbf{42.5} &\textbf{107.7} &\textbf{151.2} &\textbf{144.4}
   &\textbf{14.3} &\textbf{48.4} &\textbf{112.0} &\textbf{129.7}
   &\textbf{9.6} &\textbf{28.5} &\textbf{40.4} &\textbf{45.8}
   &\textbf{10.8} &\textbf{32.9} &\textbf{33.1} &\textbf{42.2}
\\
\hline
\hline

%%%%%%%%%%%%%%%%% right hand %%%%%%%%%%%%%%%%
{\cellcolor{white}} & {\cellcolor{white}LTD (U)~\cite{mao2019learning}}
&37.0 &82.1 &114.9 &136.1
&35.3 &79.3 &152.1 &204.3
&{22.9} &82.2 &171.7 &167.2
&25.5 &81.5 &192.9 &229.1
&45.1 &97.0 &167.7 &187.2
&25.1 &47.8 &81.0 &93.7
\\
% &Res. sup.~\cite{martinez2017human}& \\
{\cellcolor{white}} & {\cellcolor{white}DMGNN (U)~\cite{li2020dynamic}} 
&39.2  &80.5  &116.4  &129.5  
&37.5  &78.3  &156.5  &215.0 
&23.5  &85.8  &211.6  &221.4
&27.3  &83.4  &194.5  &231.0  
&47.3  &105.6 &175.6  &230.2  
&26.4  &54.2  &92.1  &103.7  
\\
{\cellcolor{white}} &{\cellcolor{white}PGBIG (U)~\cite{ma2022progressively}} 
&36.8  &78.3  &111.1  &124.6
&34.2  &76.4  &152.3  &212.5  
&24.0  &87.6  &208.3  &210.5 
&26.1  &82.5  &195.7  &233.7 
&47.2  &103.4  &173.2 &221.9
&25.7  &54.0  &91.4  &102.5 
\\
{\cellcolor{white}} & {\cellcolor{white}SPGSN (U)~\cite{li2022skeleton}} 
&33.7 &73.0 &100.0 &108.7
&\textbf{31.8} &\textbf{59.5} &146.3 &207.6
&22.5 &92.0 &213.3 &249.4
&21.3 &76.4 &185.5 &215.6
&42.4 &101.4 &166.3 &173.5
&24.7 &52.6 &89.7 &98.7
\\
\multirow{-5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{Right hands}}}
{\cellcolor{white}} &{\cellcolor{white} \textbf{EAI} (Ours)}
% &\textbf{25.2} &\textbf{59.3} &\textbf{79.3} &\textbf{74.7}
% &{32.1} &{64.3} &\textbf{100.8} &\textbf{144.8}
% &{23.8} &\textbf{72.4} &\textbf{98.0} &\textbf{96.9}
% &\textbf{21.1} &\textbf{60.4} &\textbf{147.3} &\textbf{168.0}
% &\textbf{38.4} &\textbf{69.9} &\textbf{108.8} &\textbf{122.7}
% &\textbf{21.4} &\textbf{37.9} &\textbf{70.0} &\textbf{83.5}

&\textbf{21.7} &\textbf{50.3} &\textbf{72.2} &\textbf{69.6}
&\textbf{31.8} &\textbf{70.2} &\textbf{134.0} &\textbf{180.3}
&\textbf{15.2} &\textbf{60.8} &\textbf{129.4} &\textbf{111.0}
&\textbf{17.6} &\textbf{51.0} &\textbf{116.4} &\textbf{136.9}
&\textbf{35.1} &{79.5} &\textbf{127.4} &\textbf{146.2}
&\textbf{23.1} &\textbf{46.1} &\textbf{72.0} &\textbf{86.6}
\\
\hline
\end{tabular}}
\vspace{-2.5em}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tabletex/table3_lefthand.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CA split —— AVG L, M
% 选择 A1 lift ,  A3 drink,  A5 play, A6 use, A7 on, 

\begin{table*}[t!]
\caption{Left-hand results on common action split with the evaluation metrics (in $mm$). Lower value means better performance. Obviously, our proposal outperforms all the other methods on AJME.}\
\vspace{-1em}
\label{tab:wholebody}
\centering
% \rowcolors{3}{gray!15}{white}
\resizebox{0.9\textwidth}{!}{\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{ll|cccc|cccc|cccc|cccc|cccc|cccc}

\toprule
\multicolumn{2}{c|}{Action} 
& \multicolumn{4}{c|}{A1 lift} 
& \multicolumn{4}{c|}{A2 drink} 
& \multicolumn{4}{c|}{A3 browse} 
& \multicolumn{4}{c|}{A4 use} 
& \multicolumn{4}{c|}{A5 on} 
& \multicolumn{4}{c}{A6 play}  \\
\toprule

\multicolumn{2}{c|}{Time (sec)}  & 0.2 & 0.4 & 0.8 & 1.0 & 0.8 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0 \\
\midrule

% \multirow{5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{JME}}}
{\cellcolor{white}} & {\cellcolor{white}LTD~\cite{mao2019learning}}
   &\textbf{24} &\textbf{52} &142 &211
   &21 &66 &146 &164
   &16 &\textbf{33} &126 &199
   &32 &93 &246 &304
   &11 &30 &37 &44
   &15 &35 &87 &120

\\
% &Res. sup.~\cite{martinez2017human}& \\
{\cellcolor{white}} & {\cellcolor{white}DMGNN~\cite{li2020dynamic}} 
&  &  &  &  
&  &  &  &  
&  &  &  &  
&  &  &  &  
&  &  &  &  
&  &  &  &  \\

{\cellcolor{white}} & {\cellcolor{white}SPGSN~\cite{li2022skeleton}} 
   &30 &64 &110 &160
   &20 &68 &156 &178
   &15 &36 &83 &103
   &25 &84 &256 &325
   &15 &42 &48 &55
   &16 &37 &91 &121
\\


{\cellcolor{white}} &{\cellcolor{white}PGBIG~\cite{ma2022progressively}} 
&  &  &  &  
&  &  &  &  
&  &  &  &  
&  &  &  &  
&  &  &  &  
&  &  &  &  \\
\multirow{-5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{AJME}}}
{\cellcolor{white}} &{\cellcolor{white} Ours}
   &{28} &{55} &\textbf{99} &\textbf{145}
   &\textbf{16} &\textbf{59} &\textbf{143} &\textbf{161}
   &\textbf{14} &{37} &\textbf{62} &\textbf{71}
   &\textbf{26} &\textbf{86} &\textbf{224} &\textbf{279}
   &\textbf{10} &\textbf{30} &\textbf{43} &\textbf{47}
   &\textbf{10} &\textbf{27} &\textbf{84} &\textbf{114}
\\


\bottomrule

\end{tabular}}}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tabletex/table4_righthand.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CA split —— AVG L, M
% 选择 A1 lift ,  A3 drink,  A5 play, A6 use, A7 on, 

\begin{table*}[t!]
\caption{Right-hand results on common action split with the evaluation metrics (in $mm$). Lower value means better performance. Obviously, our proposal outperforms all the other methods on AJME.}
\vspace{-1em}
\label{tab:wholebody}
\centering
\small
% \rowcolors{3}{gray!15}{white}
\resizebox{0.9\textwidth}{!}{\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{ll|cccc|cccc|cccc|cccc|cccc|cccc}

\toprule
\multicolumn{2}{c|}{Action} 
& \multicolumn{4}{c|}{A1 lift} 
& \multicolumn{4}{c|}{A2 drink} 
& \multicolumn{4}{c|}{A3 browse} 
& \multicolumn{4}{c|}{A4 use} 
& \multicolumn{4}{c|}{A5 on} 
& \multicolumn{4}{c}{A6 play}  \\
\toprule

\multicolumn{2}{c|}{Time (sec)} & 0.2 & 0.4 & 0.8 & 1.0 & 0.8 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0 \\
\midrule

% \multirow{5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{JME}}}
{\cellcolor{white}} & {\cellcolor{white}LTD~\cite{mao2019learning}}
   &37 &82 &115 &136
   &26 &82 &193 &229
   &\textbf{10} &31 &153 &218
   &30 &75 &224 &262
   &45 &97 &168 &187
   &25 &76 &126 &150

\\
% &Res. sup.~\cite{martinez2017human}& \\
{\cellcolor{white}} & {\cellcolor{white}DMGNN~\cite{li2020dynamic}} &  &  &  &  &    &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\

{\cellcolor{white}} & {\cellcolor{white}SPGSN~\cite{li2022skeleton}} 
   &31 &69 &94 &101
   &22 &80 &208 &243
   &14 &38 &68 &89
   &33 &72 &236 &284
   &46 &112 &178 &187
   &28 &81 &153 &169
\\


{\cellcolor{white}} &{\cellcolor{white}PGBIG~\cite{ma2022progressively}} &  &  &  &  &  &    &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\

\multirow{-5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{AJME}}}
{\cellcolor{white}} &{\cellcolor{white} Ours}
   &\textbf{25} &\textbf{52} &\textbf{113} &\textbf{110}
   &\textbf{22} &\textbf{68} &\textbf{165} &\textbf{188}
   &{11} &\textbf{29} &\textbf{72} &\textbf{82}
   &\textbf{25} &\textbf{57} &\textbf{204} &\textbf{243}
   &\textbf{43} &\textbf{81} &\textbf{129} &\textbf{150}
   &\textbf{20} &\textbf{55} &\textbf{104} &\textbf{123}
\\


\bottomrule

\end{tabular}}}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tabletex/table5_mainbody.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CA split —— AVG L, M
% 选择 A1 lift ,  A3 drink,  A5 play, A6 use, A7 on, 

\begin{table*}[t!]
\caption{Main-body results on common action split with the evaluation metrics (in $mm$). Lower value means better performance. Obviously, our proposal outperforms all the other methods on AJME.}
\vspace{-.5em}
\label{tab:wholebody}
\centering
\scriptsize
% \rowcolors{3}{gray!15}{white}
\resizebox{0.9\textwidth}{!}{\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{ll|cccc|cccc|cccc|cccc|cccc|cccc}

\toprule
\multicolumn{2}{c|}{Action} 
& \multicolumn{4}{c|}{A1 lift} 
& \multicolumn{4}{c|}{A2 drink} 
& \multicolumn{4}{c|}{A3 browse} 
& \multicolumn{4}{c|}{A4 use} 
& \multicolumn{4}{c|}{A5 on} 
& \multicolumn{4}{c}{A6 play}  \\
\toprule

\multicolumn{2}{c|}{Time (sec)}  & 0.2 & 0.4 & 0.8 & 1.0 & 0.8 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0 \\
\midrule

% \multirow{5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{JME}}}
{\cellcolor{white}} & {\cellcolor{white}LTD~\cite{mao2019learning}}
   &10 &21 &33 &42
   &8 &20 &45 &55
   &6 &13 &32 &44
   &12 &26 &60 &69
   &10 &18 &31 &36
   &9 &20 &33 &41

\\
% &Res. sup.~\cite{martinez2017human}& \\
{\cellcolor{white}} & {\cellcolor{white}DMGNN~\cite{li2020dynamic}} &  &  &  &  &    &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\

{\cellcolor{white}} & {\cellcolor{white}SPGSN~\cite{li2022skeleton}} 
   &13 &25 &31 &34
   &10 &22 &45 &52
   &7 &15 &26 &29
   &15 &27 &65 &77
   &13 &22 &34 &39
   &11 &22 &35 &41
\\


{\cellcolor{white}} &{\cellcolor{white}PGBIG~\cite{ma2022progressively}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\

\multirow{-5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{AJME}}}
{\cellcolor{white}} &{\cellcolor{white} Ours}
   &\textbf{10} &\textbf{20} &\textbf{30} &\textbf{34}
   &\textbf{7} &\textbf{19} &\textbf{41} &\textbf{49}
   &\textbf{6} &\textbf{12} &\textbf{25} &\textbf{28}
   &\textbf{11} &\textbf{23} &\textbf{60} &\textbf{72}
   &\textbf{8} &\textbf{15} &\textbf{26} &\textbf{31}
   &\textbf{8} &\textbf{17} &\textbf{32} &\textbf{38}
\\


\bottomrule

\end{tabular}}}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tabletex/table6_aw.tex <==
% 需要添加更多的指标,比如说拿出几个类别作为例子，剩下类别的结果放在补充材料上
\begin{table}[t!]
\caption{Average results on all actions with the evaluation metrics $MPJPE_{aw}$ (in $mm$). Lower value means better performance. Obviously, our proposal outperforms all the other methods. (Alone) represents independent training on the body parts.}
\label{tab:proto1}
\vspace{-1em}
\centering
\resizebox{0.5\textwidth}{!}{\setlength{\tabcolsep}{1mm}{
\begin{tabular}{ll|cccc|cccc}
\toprule
\multicolumn{2}{c|}{Body Parts}  & \multicolumn{4}{c|}{Left Hands} & \multicolumn{4}{c|}{Right Hands} \\
\toprule
\multicolumn{2}{c|}{Time (sec)} & 0.2 & 0.4 & 0.8 & 1.0    & 0.2 & 0.4 & 0.8 & 1.0   \\

\midrule
{\cellcolor{white}} & {\cellcolor{white}LTD~\cite{mao2019learning}}   
  
&9  &17 &34 &43
&17 &29 &50 &58
\\
% &Res. sup.~\cite{martinez2017human}& \\
{\cellcolor{white}} & {\cellcolor{white}DMGNN~\cite{li2020dynamic}}       
 
&  &  &  &    
&  &  &  &\\
{\cellcolor{white}} &{\cellcolor{white}PGBIG~\cite{ma2022progressively}} 
    
&  &  &  &    
&  &  &  &\\
{\cellcolor{white}} & {\cellcolor{white}SPGSN~\cite{li2022skeleton}}       
    
&10 &18 &35 &43
&18 &31 &50 &57
\\


\multirow{-5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{RJME}}}
& {\cellcolor{white}Ours}     
&\textbf{8} &\textbf{16} &\textbf{30} &\textbf{36}
&\textbf{15} &\textbf{27} &\textbf{44} &\textbf{50}
\\

 
\bottomrule

 

\end{tabular}}}
\end{table}

==> tabletex/table_ab.tex <==
% 需要添加更多的指标,比如说拿出几个类别作为例子，剩下类别的结果放在补充材料上

% 30 没有A（w/o MMD loss; w/o DN）
% 31 # 没有A（w MMD loss; w/o DN）
% 32 没有A（w/0 MMD loss; w DN）
% 33  没有I（w/0 Phy; w/0 S）
% 34  没有I（w/0 Phy; w S）
% 35  没有I（w Phy; w/o S）
% 30 没有A,没有I（w/o MMD loss; w/o DN）

\begin{table}[!ht]
\scriptsize
\renewcommand\arraystretch{1.2}% 行距
\centering
\vspace{-.5em}
\caption{\textbf{Ablation experiments of model architecture.} 
% DN and DC mean distribution normalization and discrepancy constraint, which are the sub-modules of XCA. PI and SI mean physical interaction and semantic interaction, which are the sub-modules of XCI. 
The best (second-best) result is highlighted in bold (underlined). }
\vspace{-1em}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|cccc|cccc|c}
\hline
 {} &{DN}&{DC} & {PI} & {SI}    &0.2s  & 0.4s  & 0.8s  & 1.0s  & Average 
\\ 
\hline
\cellcolor{white} &{} & \checkmark & \checkmark & \checkmark  &\textbf{16.7} &\textbf{40.7} &90.4 &109.8 & 64.4   
\\
\cellcolor{white}&\checkmark &  & \checkmark & \checkmark  &\underline{17.0} &41.3 &\underline{87.9} &\underline{107.1} & \underline{63.3}  
\\
\multirow{-3}{*}{{\cellcolor{white}\textbf{XCA}}}
{\cellcolor{white}} 
& &  & \checkmark & \checkmark  &\underline{17.0} &42.8 &93.7 &113.1 & 66.6  \\ 
            
\hline
\cellcolor{white}& \checkmark & \checkmark &  & \checkmark  &\textbf{16.7} &\underline{41.1} &89.8 &110.5  & 64.5  \\
\cellcolor{white}&\checkmark & \checkmark &\checkmark  &     &\underline{17.0} &42.5 &94.2 &116.1 & 67.5\\
\multirow{-3}{*}{{\cellcolor{white}\textbf{XCI}}}
&\checkmark & \checkmark &  &    &17.8 &43.2 &95.0 &118.6  & 68.7 \\
\hline
{\textbf{Full model}}&\checkmark & \checkmark & \checkmark & \checkmark  & \textbf{16.7} & \textbf{40.7} & \textbf{85.8} & \textbf{104.6} & \textbf{61.9} \\
\hline
\end{tabular}
}
\vspace{-1.em}
\label{tab:ablation}
\end{table}


==> tabletex/table_emerg.tex <==


\begin{table*}[t!]
 %\vspace{-1.em}
\caption{\textbf{The overall success rates of all skills on QUART-1 and QUART-2 with different simulation-to-real ratios. }}
\label{tab:sr}
\vspace{-1em}
\renewcommand\arraystretch{1.1}% 行距
\scriptsize
\centering
%cell大小
% \setlength{\aboverulesep}{1.85mm}
% \setlength{\belowrulesep}{-0.05mm}
\setlength{\tabcolsep}{0.42mm}{
\begin{tabular}{cc|ccc|ccc| ccc|ccc ccc|ccc|ccc|ccc}
\hline
\multicolumn{2}{c|}{\thead{Skills}} 
&\multicolumn{3}{c|}{\thead{Crawl under \textit{Bar}}} 
&\multicolumn{3}{c|}{\thead{Distinguish \textit{Letter}}}
& \multicolumn{3}{c|}{\small{\thead{Go to \textit{Object}\\and avoid the obstacle}}} 
&\multicolumn{3}{c}{\thead{Go to \textit{Object}} }
\\
\hline
\multicolumn{2}{c|}{\thead{Ratios}}  & 1:1 & 1:10 & 1:100 & 1:1 & 1:10 & 1:100 & 1:1 & 1:10 & 1:100 & 1:1 & 1:10 & 1:100       \\
\hline
& \textbf{QUART-1}

&0.74 &0.74 &0.74 
&\bf{0.46} &0.68 &0.7
&0.33 &0.60 &0.63
&0.38 &0.57 &\bf{0.71}

\\
%\hline
& \textbf{QUART-2}

&\bf{1} &\bf{1} &\bf{1} 
&0 &\bf{1} &\bf{1}
&\bf{0.7}		&\bf{0.67}		&\bf{0.9}
&\bf{0.63}		&\bf{0.7}		&0.53

\\
\hline
\multicolumn{2}{c|}{\thead{Skills}} 
&\multicolumn{3}{c|}{\thead{Go through \textit{Tunnel}}} 
&\multicolumn{3}{c|}{\thead{Stop \textit{Object}}}
&\multicolumn{3}{c|}{\thead{Unload \textit{Object}\\into \textit{Receptacle}}}
&\multicolumn{3}{c}{\thead{Average}}\\
\hline
\multicolumn{2}{c|}{\thead{Ratios}} & 1:1 & 1:10 & 1:100& 1:1 & 1:10 & 1:100& 1:1 & 1:10 & 1:100& 1:1 & 1:10 & 1:100       \\
\hline

& \textbf{QUART-1}

&\bf{0.92} &\bf{0.81} &\bf{1}
&0.17 &0.38 &0.48
&0.9 &0.94 &\bf{0.98}
&0.43 & 0.59 &0.68

\\

& \textbf{QUART-2}

&0.8		&0.7		&0.6
&\bf{0.45}		&\bf{0.8}		&\bf{0.85}
&\bf{1}		&\bf{1}		&{0.8}
&\bf{0.58}  &\bf{0.69} &\bf{0.74} 

\\
\hline

\end{tabular}
}
\vspace{-1.em}
\end{table*}


==> tabletex/table_eval.tex <==
\begin{table}[t!]
 \vspace{-.2em}
\caption{An overview of some of the evaluation scenarios used to study the emergent capabilities of QUART. They focus on three broad categories, which are (a) reasoning, (b) action
combination, and (c) quick adjustment. The visualized instructions are a subset of the full instructions}
\label{tab:evaltasks}
\vspace{-1.em}
\renewcommand\arraystretch{1.1}% 行距
\scriptsize
\centering
%cell大小
% \setlength{\aboverulesep}{1.85mm}
% \setlength{\belowrulesep}{-0.05mm}
\setlength{\tabcolsep}{0.78mm}{
\begin{tabular}{p{0.3\columnwidth}p{0.7\columnwidth}} 
\hline
\textbf{Task Group} & \textbf{Instruction} \\
\hline
Reasoning: & go to the trashcan slowly with a trotting gait \\
\hline
Reasoning: & go to the trashcan slowly with a trotting gait \\
\hline
Reasoning: & go to the trashcan slowly with a trotting gait \\
\hline
Reasoning: & go to the trashcan slowly with a trotting gait \\
\hline
Action combination: & go to the trashcan slowly with a trotting gait \\
\hline
Action combination: & go to the trashcan slowly with a trotting gait \\
\hline
Action combination: & go to the trashcan slowly with a trotting gait \\
\hline
Action combination: & go to the trashcan slowly with a trotting gait \\
\hline
Quick adjustment: & go to the trashcan slowly with a trotting gait \\
\hline
Quick adjustment: & go to the trashcan slowly with a trotting gait \\
\hline
Quick adjustment: & go to the trashcan slowly with a trotting gait \\
\hline
Quick adjustment: & go to the trashcan slowly with a trotting gait \\
\hline

\end{tabular}
}
\vspace{-1.em}
\end{table}

==> tabletex/table_exp_baseline_emergency.tex <==


\begin{table*}[t!]
 %\vspace{-1.em}
\caption{\px{\textbf{Emergency ability. Note: Citation}}}
\label{tab:exp_overall}
\vspace{-1em}
\renewcommand\arraystretch{1.2}% 行距
\scriptsize
\centering
%cell大小
\setlength{\aboverulesep}{1.85mm}
\setlength{\belowrulesep}{-0.05mm}
\setlength{\tabcolsep}{2.52mm}{
\begin{tabular}{c|c|c|c|c}
\hline

&\multicolumn{1}{c|}{\thead{CC }} 
&\multicolumn{1}{c|}{\thead{CSR}}
&\multicolumn{1}{c|}{\thead{CCP}} 
&\multicolumn{1}{c}{\thead{Average}}
\\
\hline
% \multicolumn{2}{c|}{\thead{Ratios}}  & 1:1 & 1:10 & 1:100 & 1:1 & 1:10 & 1:100 & 1:1 & 1:10 & 1:100 & 1:1 & 1:10 & 1:100       \\
{CLIP}\cite{radford2021learning}&
0.74  &0.74 &\bf{0.46}   &\bf{0.46} \\
{R3M}\cite{nair2022r3m}
&0.74  &0.74 &\bf{0.46}  &\bf{0.46}\\
{VC-1}\cite{vc2023}
&0.74  &0.74 &\bf{0.46}&\bf{0.46} \\
{QUART-1}
&\bf{1} &0.74 &\bf{1} &\bf{0.46} \\
\textbf{QUART-2}
&\bf{1} &0.74  &\bf{1} &\bf{0.46} \\
\hline

\end{tabular}
}
\vspace{-1.em}
\end{table*}


==> tabletex/table_exp_baseline_unseen.tex <==


\begin{table*}[t!]
 %\vspace{-1.em}
\caption{\px{\textbf{Unseen tasks on Baselines. Note: Citation}}}
\label{tab:exp_unseen}
\vspace{-1em}
\renewcommand\arraystretch{1.2}% 行距
\scriptsize
\centering
%cell大小
% \setlength{\aboverulesep}{1.85mm}
% \setlength{\belowrulesep}{-0.05mm}
% \setlength{\tabcolsep}{0.42mm}{
\begin{tabular}{cc|c|c|c|c|c|c|c|c }
\hline
\multicolumn{2}{c|}{\thead{}} 
&\multicolumn{1}{c|}{\thead{Skills}} 
&\multicolumn{1}{c|}{\thead{Distinguish}}
&\multicolumn{1}{c|}{\thead{Go to} }
& \multicolumn{1}{c|}{\thead{Go avoid}}
&\multicolumn{1}{c|}{\thead{Go through}} 
% &\multicolumn{1}{c|}{\thead{Stop}}
&\multicolumn{1}{c|}{\thead{Crawl}} 
&\multicolumn{1}{c|}{\thead{Unload}}
&\multicolumn{1}{c}{\thead{Average}}
\\
\hline
% \multicolumn{2}{c|}{\thead{Ratios}}  & 1:1 & 1:10 & 1:100 & 1:1 & 1:10 & 1:100 & 1:1 & 1:10 & 1:100 & 1:1 & 1:10 & 1:100       \\


{}&&{CLIP}\cite{radford2021learning}
& 0.52  & 0.41 & 0.44 & &0.04  && \\

{}&&{R3M}\cite{nair2022r3m}
&  &  &  & &  & & \\
{}&&{VC-1}\cite{vc2023}
&  &  &  & &  & & \\

{}&&{QUART-1}
&  &  &  & &  & & \\

\multirow{-5}{*}{\rotatebox[origin=c]{90}{{ \textbf{Texture}}}}
&&\textbf{QUART-2}
& 0.52 & 0.4 & 0.55 & &0.26  & & \\


\hline

{}&&{CLIP}\cite{radford2021learning}
& &   0.42& 0.42 & &  & & \\

{}&&{R3M}\cite{nair2022r3m}
&  &  &  & &  & & \\
{}&&{VC-1}\cite{vc2023}
&  &  &  & &  & & \\

{}&&{QUART-1}
&  &  &  & &  & & \\

\multirow{-5}{*}{\rotatebox[origin=c]{90}{{ \textbf{Object}}}}
&&\textbf{QUART-2}
&  & 0.54 & 0.50  & &  & & \\


\hline

% \hline

% {}&&{CLIP}&
% 0.74  &0.74 &\bf{0.46} &0.68  &0.74  &\bf{0.46} &\bf{0.46} \\

% {}&&{R3M}
% &0.74  &0.74 &\bf{0.46} &0.68  &0.74  &\bf{0.46} &\bf{0.46} \\
% {}&&{VC-1}
% &0.74  &0.74 &\bf{0.46} &0.68  &0.74  &\bf{0.46} &\bf{0.46} \\

% {}&&{QUART-1}
% &\bf{1} &0.74 &\bf{1} &\bf{1}  &0    &\bf{0.46}&\bf{0.46}  \\

% \multirow{-5}{*}{\rotatebox[origin=c]{90}{{ \textbf{Verbal}}}}
% &&\textbf{QUART-2}
% &\bf{1} &0.74  &\bf{1} &\bf{1}    &0.74  &\bf{0.46}&\bf{0.46}  \\


% \hline
\end{tabular}
% }
\vspace{-1.em}
\end{table*}


==> tabletex/table_exp_speed.tex <==


\begin{table*}[t!]
 %\vspace{-1.em}
\caption{\px{\textbf{Inference speed.}}}
\label{tab:exp_speed}
\vspace{-1em}
\renewcommand\arraystretch{1.2}% 行距
\scriptsize
\centering
%cell大小
% \setlength{\aboverulesep}{1.85mm}
% \setlength{\belowrulesep}{-0.05mm}
% \setlength{\tabcolsep}{0.42mm}{
\begin{tabular}{cc|c|c|c|c|c|c |c|c|c }

\\
\hline
\multicolumn{2}{c|}{\thead{Split}} 
&\multicolumn{3}{c|}{\thead{Slowly}} 
&\multicolumn{3}{c|}{\thead{Normally}}
& \multicolumn{3}{c}{\thead{Quicly}}

\\
\hline
\multicolumn{2}{c|}{\thead{Skills}} 
&\multicolumn{1}{c|}{\thead{Go to}} 
&\multicolumn{1}{c|}{\thead{Go Avoid}} 
&\multicolumn{1}{c|}{\thead{Crawl}}
&\multicolumn{1}{c|}{\thead{Go to}} 
&\multicolumn{1}{c|}{\thead{Go Avoid}} 
&\multicolumn{1}{c|}{\thead{Crawl}}
&\multicolumn{1}{c|}{\thead{Go to}} 
&\multicolumn{1}{c|}{\thead{Go Avoid}} 
&\multicolumn{1}{c}{\thead{Crawl}}
\\
\hline
% \multicolumn{2}{c|}{\thead{Ratios}}  & 1:1 & 1:10 & 1:100 & 1:1 & 1:10 & 1:100 & 1:1 & 1:10 & 1:100 & 1:1 & 1:10 & 1:100       \\
{{CLIP}\cite{radford2021learning}}&
&0.44 & 0.43 & 0.45& 0.19& 0 & 0\\

{R3M}\cite{nair2022r3m}&
& & & & &  \\
{VC-1}\cite{vc2023}&
& & & & &   \\

\textbf{QUART-1}&
& & & & &   \\

\textbf{QUART-2}&
&\textbf{0.66}  &\textbf{0.60}& \textbf{0.53}& \textbf{0.41}& \textbf{0.32}\\

\hline

\end{tabular}
% }
\vspace{-1.em}
\end{table*}


==> tabletex/table_seen.tex <==
\newcommand{\seen}[1]{\textcolor{blue}{#1}}
\newcommand{\unseen}[1]{\textcolor{red}{#1}}


\begin{table*}[h]
  \setlength\tabcolsep{2.3pt}
  \centering
  % \hspace*{-1.9cm}
  \scriptsize
\begin{tabular}{lcccccccccccccccccccccccc}
\toprule
 Method  &\multicolumn{1}{c}{\thead{crawl-\\\seen{seen}-red-bar}} 
 & \multicolumn{1}{c}{\thead{distinguish-\\\seen{seen}-letter-d}} 
 & \multicolumn{1}{c}{\thead{go avoid-\\\seen{seen}-cooker}}  
 & \multicolumn{1}{c}{\thead{go avoid-\\\seen{seen}-drawers}} 
 & \multicolumn{1}{c}{\thead{go avoid-\\\seen{seen}-oven}} 
  & \multicolumn{1}{c}{\thead{go avoid-\\\seen{seen}-table}} 
\\
      \midrule
QUART-1 &0.7 & 0.7  & 0.5 & 0.29 & 0.48  & 0.34 \\
QUART-2 &\bf{1} &\bf{1}  &\bf{1} & \bf{0.80}  & \bf{1}  &\bf{1}    \\

\toprule
 Method  
  & \multicolumn{1}{c}{\thead{go to-\\\seen{seen}-chair}}
 & \multicolumn{1}{c}{\thead{go avoid-\\\seen{seen}-vase}}
 &\multicolumn{1}{c}{\thead{go through-\\\seen{seen}-rectangle-tunnel}} 
 &\multicolumn{1}{c}{\thead{go through-\\\seen{seen}-triangle-tunnel}} 
 
 & \multicolumn{1}{c}{\thead{stop-\\\seen{seen}-purple-ball}} 
 & \multicolumn{1}{c}{\thead{go avoid-\\\seen{seen}-pink-ball}}  

 & \multicolumn{1}{c}{} 

 \\  
      \midrule
QUART-1 & 0.38 & 0.56 &0.8 &0.96  & \bf{0.2} & 0.72      &  & \\
QUART-2 & \bf{0.4} & \bf{0.6} &\bf{1} & \bf{1}    & 0.1 & \bf{1}      &   &        \\



 \bottomrule
\end{tabular}
  \vspace{0.5em}
  \caption{\px{need to be added}Overall Performance
  }
\label{table:seen}
\end{table*}

==> tabletex/table_split.tex <==
% % 需要添加更多的指标,比如说拿出几个类别作为例子，剩下类别的结果放在补充材料上
% \begin{table*}[t!]
% \caption{Average results on all actions with the evaluation metrics (in $mm$). Lower value means better performance. Obviously, our proposal outperforms all the other methods. (Alone) represents independent training on the body parts.}
% \label{tab:proto1}
% \vspace{-1em}
% \centering
% \resizebox{0.96\textwidth}{!}{\setlength{\tabcolsep}{1mm}{
% \begin{tabular}{ll|cccc|cccc|cccc|cccc|cccc|cccc|cccc}
% \toprule
% \multicolumn{2}{c|}{Body Parts} & \multicolumn{4}{c|}{Main body} & \multicolumn{4}{c|}{Left Hands} & \multicolumn{4}{c|}{Right Hands} & \multicolumn{4}{c|}{Whole Body} & \multicolumn{4}{c|}{Main body (Alone)} & \multicolumn{4}{c|}{Left Hands (Alone)} & \multicolumn{4}{c}{Right Hands (Alone)}\\
% \toprule
% \multicolumn{2}{c|}{Time (sec)} & 0.2 & 0.4 & 0.8 & 1.0    & 0.2 & 0.4 & 0.8 & 1.0    & 0.2 & 0.4 & 0.8 & 1.0   & 0.2 & 0.4 & 0.8 & 1.0    & 0.2 & 0.4 & 0.8 & 1.0    & 0.2 & 0.4 & 0.8 & 1.0 & 0.2 & 0.4 & 0.8 & 1.0\\

% \midrule
% {\cellcolor{white}} & {\cellcolor{white}LTD~\cite{mao2019learning}} 
%  &9 &20 &41 &50
%  &20 &50 &123 &162
%  &32 &75 &157 &195
%  &18 &43 &95 &120
 
%  &9  &20  &42  &51 
%  &20  &57  &143  &181     
%  &33  &77  &159  &195\\

% % &Res. sup.~\cite{martinez2017human}& \\
% {\cellcolor{white}} & DMGNN~\cite{li2020dynamic}  
% &  &  &  &     
% &  &  &  &    
% &  &  &  & 
% &  &  &  &
% &  &  &  &    
% &  &  &  &     
% &  &  &  &\\
% {\cellcolor{white}} &{PGBIG~\cite{ma2022progressively}} 
% &  &  &  &      
% &  &  &  &     
% &  &  &  &     
% &  &  &  & 
% &  &  &  &     
% &  &  &  &     
% &  &  &  &\\
% {\cellcolor{white}} & {SPGSN~\cite{li2022skeleton}}   
% &13 &25 &44 &53 
% &22 &56 &125 &161
% &34 &75 &152 &191
% &21 &47 &96 &120 
% &  &  &  &     
% &  &  &  &     
% &  &  &  &\\




% \multirow{-5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{AJME}}}

% & {\cellcolor{white}Ours} &\textbf{8} &\textbf{18} &\textbf{38} &\textbf{46}
% &\textbf{18} &\textbf{49} &\textbf{108} &\textbf{135}
% &\textbf{31} &\textbf{69} &\textbf{139} &\textbf{166}
% &\textbf{17} &\textbf{40} &\textbf{85} &\textbf{103}
% &  &  &  &     &  &  &  &     &  &  &  &\\





% \midrule
% {\cellcolor{white}} & {\cellcolor{white}LTD~\cite{mao2019learning}}   
% & - & - & - & -  
% &9  &17 &34 &43
% &17 &29 &50 &58
% & - & - & - &  -
% &  &  &  &     
% &  &  &  &     
% &  &  &  &\\
% % &Res. sup.~\cite{martinez2017human}& \\
% {\cellcolor{white}} & {\cellcolor{white}DMGNN~\cite{li2020dynamic}}       
% & - & - & - & -    
% &  &  &  &  
% &  &  &  &
% & - & - & - &  -
% &  &  &  &    
% &  &  &  &    
% &  &  &  &\\
% {\cellcolor{white}} &{\cellcolor{white}PGBIG~\cite{ma2022progressively}} 
% & - & - & - & -    
% &  &  &  &  
% &  &  &  &
% & - & - & - &  -
% &  &  &  &     
% &  &  &  &    
% &  &  &  &\\
% {\cellcolor{white}} & {\cellcolor{white}SPGSN~\cite{li2022skeleton}}       
% & - & - & - & -    
% &10 &18 &35 &43
% &18 &31 &50 &57
% & - & - & - &  -
% &  &  &  &     
% &  &  &  &     
% &  &  &  &\\


% \multirow{-5}{*}{\rotatebox[origin=c]{90}{\cellcolor{white}\textbf{RJME}}}
% & {\cellcolor{white}Ours}     
% & - & - & - & -    
% &\textbf{8} &\textbf{16} &\textbf{30} &\textbf{36}
% &\textbf{15} &\textbf{27} &\textbf{44} &\textbf{50}
% & - & - & - &  -
% &  &  &  &     
% &  &  &  &     
% &  &  &  &\\

 
% \bottomrule

 

% \end{tabular}}}
% \end{table*}
